PyGlove: Efficiently Exchanging ML Ideas as Code

The increasing complexity and scale of machine learning (ML) has led to the need for more efficient collaboration among multiple teams. For example, when a research team invents a new architecture like "ResNet," it is desirable for multiple engineering teams to adopt it. However, the effort required for each team to study and understand the invention does not scale well with the number of teams or inventions. In this paper, we present an extension of our PyGlove library to easily and scalably share ML ideas. PyGlove represents ideas as symbolic rule-based patches, enabling researchers to write down the rules for models they have not seen. For example, an inventor can write rules that will "add skip-connections." This permits a network effect among teams: at once, any team can issue patches to all other teams. Such a network effect allows users to quickly surmount the cost of adopting PyGlove by writing less code quicker, providing a benefit that scales with time. We describe the new paradigm of organizing ML through symbolic patches and compare it to existing approaches. We also perform a case study of a large codebase where PyGlove led to an 80% reduction in the number of lines of code.

==> src/rebuttal/1_introduction.tex <==
\section{Introduction}\label{sec:introduction}

Thousands of machine learning (ML) papers are submitted each year to top-tier conferences and journals.
Many of these venues now encourage the open-sourcing of relevant code, such as NeurIPS or ICLR, highlighting the need for researchers and practitioners to share not only their ideas but also their implementation.
This is true within organizations too, which today can employ thousands. In particular, the training and deployment of large models now require multiple engineers and researchers to work together. Whether within a large group or the ML community as a whole, exchanging code to keep up with discoveries is essential.
For example, image classification has seen in recent years transitions from plain convolutional networks, to the introduction of batch normalization~\cite{ioffe2015batch}, residuals~\cite{he2016deep}, inverted bottlenecks~\cite{sandler2018mobilenetv2}, and a transition to transformers~\cite{vaswani2017attention}.
A team working on image classification that wants to keep their models up to date would have had to incorporate these changes either by adapting the external code through interfaces or simply rewriting it -- both time-consuming processes.
This is challenging because different teams develop their own conventions without any unifying standards. Our paper addresses this problem by extending {\NAME}~\cite{peng2020pyglove} to a language that allows defining flexible standards and writing rules for how to use the standards to exchange code easily.

Flexibility is key, as enforcing strict standards may limit long-term progress. This is because it can be difficult to avoid over-emphasizing our current ideas when defining conventions. For example, in 2015, we may have adopted an interface in which every layer receives only the activations of the previous layer, so in 2016 we would have had to rewrite our interface to include the skip-connections of a ResNet. Another example would have been to assume independence across examples at training time, which would need to be broken to apply batch-normalization. In each case, we made an assumption that was later broken by new discoveries. One possible solution is to simply accept that standards must evolve \cite{sussman2007building}. Thus, our approach allows defining editable standards.

To achieve these goals, {\NAME} takes a rule-based approach: standards are first defined by light-weight annotations of ML code and then rules indicate how the code should be shared. For example, consider a situation in which ``team A'' maintains an image classifier and ``team B'' independently comes up with a new convolutional layer that should improve most image classifiers. In the {\NAME} approach, team A can annotate their (pre-existing) code with statements akin to ``this is a convolution'', ``this is a nonlinearity'', and so on, and team B would annotate their new layer with statements akin to ``these are hyperparameters'' (see \Secref{sec:symbolic-patching}).
Up to this point in our example, the two teams need not have interacted at all. Upon team A learning about the new layer, A can write a one-line rule equivalent to ``replace all my convolutions with team B's layer'' (technically accurate examples in \Secref{sec:symbolic-patching}).
Additionally, {\NAME} also allows a novel twist: team B can write the replacement rule themselves -- such a rule would be analogous to ``in any image classifier, replace all convolutions with our layer''. Then any team with a {\NAME}-annotated image classifier can apply the rule produced by team B. This twist opens up future collaboration options through repositories of ML inventions, which we discuss in \Secref{subsec:patch-power}.

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-5mm}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{src/figures/network_effects_v3.pdf}
  \end{center}
  \label{fig:network-effects}
\vspace{-4mm}
\caption{
Applying $m$ new ML innovations to $n$ teams leads to $n{\times}m$ code changes.
{\NAME} expresses an ML innovation as a sharable rule that can be applied at once by each of the $m$ teams.
% Network effect among ML ideas: with existing ideas (expressed by rule -- a block), introducing a new idea can lead to an exponential growth of the applications of these ideas.
%
% A single additional patching rule (\#N+1) leads to 
%
%more than O(N) different kinds of experiments.
% 6 patching rules leads to 9 unique valid object detection experiments. Adding an experiment will double the number, creating a network effect.
}
\end{wrapfigure}
PyGlove's rule-based approach is not constrained to the sharing of architectural changes but applies to all aspects of the ML pipeline, such as data augmentation, training algorithm, or meta-learning. In particular, as ML hardware improves, there is a recurring need to scale up model capacity. Empirical and theoretical rules have been invented to address this problem~\cite{sussman2007building,tan2019efficientnet,yang2021tuning}. Such rules could be broadcasted throughout an organization or the community, saving valuable engineer time.
% Moreover, network effects are possible by combining these rules.
This is true even across codebases, provided the guidelines in \Secref{subsec:scale-ml-network-effect} are followed. \Figref{fig:network-effects} illustrates the efficiency gains through community network effects: without PyGlove $m$ innovations applied to $n$ team projects result in $m \times n$ work; with PyGlove, each innovation requires writing a PyGlove rule ($m$ rules) and each team project is responsible for PyGlove annotations in their own model ($n$ models), resulting in only $m + n$ work, as the rule application is trivial.
In addition to the sharing of code, {\NAME}'s rules can also allow an individual to manipulate their ML system. In all these cases, our rule-based approach stands in contrast to current methods, which typically require multiple in-place edits that do not scale well with the size of the model or with the number of practitioners in the community.
These comparisons are detailed in \Secref{sec:pyglove-analysis}.\looseness=-1



The reason why {\NAME} can be applied broadly to all aspects of ML code -- and indeed beyond ML -- is its principled symbolic programming design~\cite{mccarthy1960recursive}.
Under this paradigm, {\NAME}-annotated Python objects become editable symbols, and {\NAME} rules are meta-programs that act on these symbols.
The rules are also symbols themselves, allowing compositionality similar to that of a LISP program's ability to self-edit~\cite{steele1990common}.
In \Secref{sec:symbolic-program-ml}, we describe symbolic programming and explain the {\NAME} design.\looseness=-1

To summarize, our contributions are:
\begin{itemize}
    \item A novel annotation-based language to express flexible standards that can evolve over time;
    \item A principled, rule-based method for easily exchanging complex ML ideas as code;
    \item Guidelines for efficient {\NAME} usage across large teams or communities; and
    % \item a formalization of allowing programs to modify programs at runtime for ML.
    % \item a formalization of {\NAME}'s programming paradigm for ML
    \item A formulation of ML's life-cycle through a symbolic programming paradigm.
    % for machine learning.
    % \item a formalization of our method as symbolic programming for machine learning.
\end{itemize}

The final product, {\NAME}, is open-sourced with this paper.
%at GitHub \url{https://github.com/google/pyglove}.


==> src/rebuttal/2_method.tex <==
\section{Expressing ML Ideas Through Patching }\label{sec:symbolic-patching}

The engineering process of ML is to journey from experiment A to experiment B, in which an iteration is made by manually applying the conceptual rules that formulate an idea to an ML program---a process of source code manipulation.
For example, supposing an ML practitioner wants to swap all the convolution layers with separable convolution layers in a neural network, the practitioner must locate the appearances of all convolution units in the model source code and replace each of them with the intended separable convolution.
To automate this process, we need the ML program to be manipulated programmatically. 
Such program modification is not only necessary to implement an idea but required to apply the same idea to other ML programs without complicating their codebases.
% A natural intuition is to allow an ML program to be dynamically modifiable at run time, which has been long offered by a symbolic programming paradigm originated from LISP~\cite{steele1990common}, later introduced to AutoML by {\NAME}\cite{peng2020pyglove}. Here we extend {\NAME}'s symbolic capacity from AutoML~\cite{peng2020pyglove} to ML, to express the rules embodied in the previous manual process and encapsulate them into reusable program units across different ML programs.
A natural intuition is to allow an ML program to be dynamically modifiable at run time. Motivated by this, we develop {\NAME} to express the rules embodied in the previous manual process and encapsulate them into reusable program units across different ML programs.
% ~\cite{hutchins1985direct}
As a result, not only a complex idea can be implemented by directly manipulating the ML programs, but also the laborious repetition of daily ML practices can be captured by such program expression of rules -- \emph{patches}.
The use case mentioned above in which team A applies team B's latest convolution invention without laborious manual coding is illustrated in \Figref{fig:symbolic_exp_sim_v1}.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\textwidth]{src/figures/patch_overview_v2.pdf}
    \includegraphics[width=0.9\textwidth]{src/figures/first_patch_simple_example_v4.pdf}
    \caption{
Team B's new invention \TT{SepConv} is developed agnostic to Team A's experiment, but its rule \TT{apply\_sepconv} can be patched to upgrade Team A's experiment into \TT{new\_resnet}.
In this code, \TT{pg.symbolize} is the annotation that adds the editable trait to regular Python classes, and \TT{pg.patch} is the operation that applies a rule to an object of an annotated class.
}
    \label{fig:symbolic_exp_sim_v1}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth]{src/figures/symbolic_exp_complex_v2.pdf}
    \caption{
Three more complex ideas are expressed via {\NAME} patching rules.
(Left) To change the dataset for a classification task, we need to change both the dataset and the model header's width to align with the number of classes.
This is done by querying the location of the last Dense layer, and returning the new value for both the dataset and the dense units associated with their locations as an update to the experiment.
(Middle) To multiply a scaling factor on the channels of the Conv and FC layer, the patching rule is defined by a function for transforming each node in the object tree, which takes the location, value and parent of current node as input, and modifies the `channels' member of Conv and FC classes. (Right) A upgraded version of previous example, which uses AutoML for scaling the model with a target FLOPs. To do so, it generates a search space of scale factors, and connects the search space to an AutoML trainer, which automatically figure out the best choices.
% based on the target flops.
}
    \label{fig:symbolic_exp_complex_v1}
\end{figure}






\subsection{The Power and Compositionality of Patching}   \label{subsec:patch-power}



\begin{wrapfigure}{r}{0.32\textwidth}
  \vspace{-6mm}
  \begin{center}
    \includegraphics[width=0.32\textwidth]{src/figures/patch_composition_v3.pdf}
  \end{center}
\vspace{-4mm}
\caption{
The LaMDA paper~\cite{thoppilan2022lamda} can be obtained by applying a composition of patches on the Transformer paper~\cite{wolf2020transformers}.
}
\vspace{-5mm}
\label{fig:patch_composition}
\end{wrapfigure}
The simplicity of {\NAME} to express rules is also applicable to more complex ideas.
With a capacity of direction manipulation~\cite{hutchins1985direct}, the user can modify program parts in an ML experiment by locations or by rules.
For example, \Figref{fig:symbolic_exp_complex_v1} illustrates how to change dataset, scale the width of neural models, and automatically scale the model by AutoML through {\NAME}.


% Patches themselves are symbolic objects \daiyip{Can we use it and refer to later section without definition?}(See \Secref{}), which can be serialized and moved across codebases and processes.

Simple patches can be combined together to express complex ideas.
For example, the recent large-scale NLP algorithm, LaMDA~\cite{thoppilan2022lamda}, can be obtained by applying common patches to the Transformer paper~\cite{wolf2020transformers}.
We briefly introduced how this can be implemented with {\NAME} in \Figref{fig:patch_composition}. 


Patches, i.e., program expression of rules, are useful not only because they make the expression of ideas straightforward but also because they can be shared freely and applied to different ML experiments.
{\NAME} allows patches themselves to be easily shared across codebases.
It allows users to create a patch from a URI-like string, which is human readable and can be easily referred to with a global unique name. For example, a patch for changing dataset to ImageNet~\cite{deng2009imagenet} can be described as \TT{``change\_dataset?name=imagenet''}.



% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-10mm}
%   \begin{center}
%     \includegraphics[width=0.45\textwidth]{xfigures/patch_network_effect_v1.pdf}
%   \end{center}
% \vspace{-4mm}
% \caption{
% 6 patching rules leads to 9 unique valid object detection experiments. Adding an experiment will double the number, creating a network effect.
% }
% \vspace{-1mm}
% \label{fig:patch_network_effect}
% \end{wrapfigure}


\begin{wrapfigure}{r}{0.58\textwidth}
  \vspace{-6mm}
  \begin{center}
    \includegraphics[width=0.58\textwidth]{src/figures/deep_network_effect_v4.pdf}
  \end{center}
\vspace{-4mm}
\caption{
Without {\NAME}, patching $m$ changes into $n$ teams requires $n\times{m}$ modifications to the code.
With {\NAME}, each $A_{i}$ team annotates their own code and each $B_{j}$ team writes their own rules.
As a result, patching all changes takes $n+m$ changes only.
}
\vspace{-8mm}
\label{fig:deep_network_effect}
\end{wrapfigure}
The compositionality of patches leads to a network effect among the ML ideas. We illustrate a common scenario in \Figref{fig:deep_network_effect}, that how research teams (Teams $B_{i}$) share their latest discoveries with product teams (Teams $A_{i}$). Based on {\NAME}, a research discovery can be encapsulated by a patching rule. Once the rule is created, any product team whose codebases are annotated by {\NAME} in a compatible way can apply it. This means that a research team's idea can be adopted by many product teams without manually integrating it each time. Similarly, a product team can try many research ideas quickly. This has not yet count the combination of patches, which can grow the degree of network effect exponentially. 


%\tododp{Revise the words to align with the new figures.}
% As illustrated in \Figref{fig:network-effects}, we have $3$ patching rules for data augmentation policies and $3$ patching rules for learning schedules.
% Then, we can get $3*3=9$ different experiments through combination, even if the learning schedules are mutually-exclusive and augmentation policies are also exclusive.
% Furthermore, when we add an experiment, for example, an image classification task, it will double the number of valid combinations. Therefore, once we have a fair amount of patching rules and experiments, the variety of valid experiments that can be expressed can grow exponentially.

% \tododxy{can you add a diagram here to illustrate the network effect described above?} # DONE

\subsection{Scaling Up the Network Effect of ML Ideas}\label{subsec:scale-ml-network-effect}

Patches need to be written wisely. For example, consider the following potential pitfall: assuming a research team has found a brilliant way to figure out the learning rate for image classifiers, they write a rule depending on a ``\TT{learning\_rate}'' property of the task after seeing it fit for an \TT{ImageClassificationTask} class.
Later someone in this team wants to apply the rule to another image classifier - \TT{ImgClsTask}, which, instead of having \TT{``learning\_rate''}, has a \TT{``lr''} property. The rule will surely fail due to the mismatch between the expected and actual locations for the learning rate. In such case, a better rule can be written as - matching any node under the task whose key is either \TT{``learning\_rate''} or \TT{``lr''}, which not only work for the cases above, but also for cases that specifies learning rate not as an immediate property of the task, but under its sub-node such as an optimizer.
This approach, however, does not scale well since the pre-defined assumptions cannot always meet the growth of heterogeneous components. As a result, to maximize the generality of rules, we need to reduce the discrepancies among ML components by advocating reuse at both the low level (e.g., network layers) and higher levels (e.g., training loop definition).

Standardization is the process of reducing the applicability issues for patching across codebases. It sounds alarming, as usually, standardization means reducing flexibility and autonomy.
In our proposal, however, we suggest an ML component ecosystem that carefully considers the flexibility and self-govern needs, while allowing different codebases to converge in what ML components they use incrementally. Such an ML ecosystem should have the following requirements:

\textbf{(1) Concept-oriented} Components in the ML ecosystem should precisely represent the concepts in the human mind. They should be able to be put together by composition and can be manipulated easily. ML components like this should allow a natural mapping of the concepts and straightforward expressions of ideas, which makes them competitive for broad adoption.


\textbf{(2) Scalable for extension} The components should be extensible without modifying the existing source code.
In other words, a component can be extended without modifying its class definition, and an object of the component should be able to be modified without changing its source code.

\textbf{(3) Runtime independence} The user-facing interfaces should be independent of the execution environment, such as ML frameworks, hardware accelerators, etc.
If so, it will allow the identical ML experiment definition to run consistently from everywhere.

\textbf{(4) Maximizing sharing} Both ML components and their objects can be easily shared. Moreover, ML objects of common interests, such as well-known experiments, can be retrieved with a globally unique identifier (e.g., URL), which automatically imports their required components.
Therefore, ML experiments and techniques can be easily referenced by their identifiers.

\textbf{(5) Adaptive to changes} The ML ecosystem needs to adapt to the rises and falls of standard components.
This requires a scalable way of upgrading the existing experiments with new components that replaces the old components.

\textbf{(6) Supporting accessibility} The advocate for sharing does not mean that everything needs to be public. Organizations or individuals are welcome to have their own assets, no matter it is IP reasons or certain assets are too early to be shared publicly. Accessibility can be controlled at both component level and object level.

{\NAME} provides solutions to all these requirements:
\begin{itemize}
    \item A PyGlove-annotated object is a straightforward solution for developing concept-oriented components, which is compositional and mutable, addressing requirement (1).
    \item A PyGlove-annotated class can be extended by subclassing, and its object can be modified with manipulation, satisfying requirement (2).
    \item Patches can be easily developed to map common PyGlove-annotated classes to their runtime-specifc versions. Therefore, the user-facing components are decoupled completely from the components for implementation, meeting requirement (3).
    \item PyGlove-annotated objects are serializable, which can be stored in a file or database. Moreover, the serialized information contains the information for importing their components, so users can load the object through a single URL, addressing requirement (4).
    \item Upgrading an old component in existing experiments can be described as a patch, which can be triggered periodically on existing experiments, meeting requirement (5).
    \item Requirement (6) can be achieved easily with existing source control solutions.
\end{itemize}

%
% \tododxy{can you please insert a figure for supporting runtime independence?}
%\subsection{An Ultimate Goal}


% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-7mm}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{xfigures/final_picture_v1.pdf}
%   \end{center}
% \vspace{-3mm}
% \caption{
% The experiment of the LaMDA\cite{} paper can be be described as a previous experiment combined with existing or new techniques.
% }
% \vspace{-6mm}
% \label{fig:final_picture}
% \end{wrapfigure}



==> src/rebuttal/3_symbolic_ml.tex <==


\section{Symbolic Programming for Machine Learning}\label{sec:symbolic-program-ml}


Patching demonstrates a unique angle to view machine learning programs through a lens of symbols, which directly maps the concepts from the human mind to computer program expressions~\cite{sussman2007building}. Symbolic programming, however, has a much broader usage in the entire life-cycle of ML than just patching. Before we get to that point, let's take a brief look at what symbolic programming is, why we need it in ML and PyGlove's offering about it.

Symbolic programming, which originated from \cite{steele1990common}, is a programming paradigm to manipulate its own components as if they were plain data~\cite{mccarthy1960recursive}.
Symbolic programming is interesting to ML since ML is overloaded with a constant need for modifying the source code of  ML programs.
It accommodates the ideas that can not be done with predefined interfaces and frequently changed hyperparameters. When rules are introduced to change the behavior of programs, they either need to change the source code or manipulate them at run time. The former is not viable for ML, since ML requires different experiments to be obtained from the same source code. The other option seems to be a more flexible solution to try. Have we considered code generation?
Of course, manipulation has to be done with code generation at run time. But what about generating source code?
Our answer is no.
It is neither easy nor flexible, because (1) it requires templates for the source code, which are not generally applicable to all existing code, and (2) it is difficult to accommodate complex manipulation patterns, such as mutate-run-mutate, which is commonly needed in ML. For example, in \Figref{fig:symbolic_exp_complex_v1}-1, to change the dataset for an ML classifier, we need to generate code for loading that dataset by a name, evaluate it to get the number of classes for the task, and then apply the number to generate the code of the model head width.


\subsection{PyGlove's Symbolic Programming Solution}


PyGlove formulates its symbolic programming solution through the concept of symbolic object.
A symbolic object is a unity of symbol and object, with the two aspects synchronized, meaning that \textit{a symbolic object can be manipulated as a symbol, while it can be evaluated as a regular object}.
A symbolic object is an instance of a symbolic class, which can be created by annotation \TT{pg.symbolize}, illustrated in \Figref{fig:symbolic_ops}(1). While the class can be used as a regular class, this tiny decorator makes the operations illustrated in \Figref{fig:symbolic_ops}(2-8) applicable to its objects. Symbolic object has many characteristics: first of all, the construction information (type, constructor arguments) is preserved, which defines its \emph{symbolic representation}. Such representation is identical between its source form and run-time form, thus carries necessary information to fully embody the concept that the object represents. As a result, such representation is a proxy to the concept for manipulations - ideas can be expressed as direct manipulation~\cite{hutchins1985direct} of concepts through their symbolic representations. On the other hand, a symbolic object is also a program entity that exists at run time, which carries data members and methods, behaving like a regular object. The unity of being symbolic and being an object allows a symbolic object to take advantage of the capabilities from both object-oriented programming and symbolic programming, while the former allows a modular and extensible software design, the latter brings the power of meta-programming through manipulations.


\begin{figure}[h!]
    %\vspace{-5mm}
    \centering
    \includegraphics[width=0.90\textwidth]{src/figures/ml_symboy_ops_v1.pdf}
    \caption{The definition of a symbolic class, its instance (an symbolic object), and common symbolic operations that can be applied on it. A symbolic object can be developed, validated, inspected, compared, cloned, serialized, mutated, place-held and generated with ease.}
    \label{fig:symbolic_ops}
    \vspace{-1mm}
\end{figure}



\subsection{How Symbolic Object Serves Machine Learning End-to-End}


%Now we take a breadth-first view at how PyGlove serves the life-cycle of ML. \Figref{fig:symbolic_ops} shows the symbolic operations that are used during daily ML workflows. Through \Figref{fig:ml_cycle}, we demonstrate the combination of such operations can effectively address the requirements from different phases of the ML life-cycle, from reproduction to release.

Let us take a closer look at how symbolic objects serve ML.
First, the mutability of symbolic object removes the need for hyperparameter containers, which makes the development and use of ML components much simpler and more consistent. Second, the combination of symbolic operations can effectively address the need of ML experimentation with a few lines of code. \Figref{fig:ml_cycle} illustrates the symbolic operations involved in the ML life-cycle based on the \TT{MLExperiment} class defined in \Figref{fig:symbolic_ops}.\looseness=-1




\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{src/figures/ml_experiment_cycle_v4.pdf}
    \caption{
    {\NAME} serves the ML life-cycle.
    {\NAME} simplifies the engineering efforts involved from the birth of a research idea to its graduation while making the whole or parts of an experiment reusable.\looseness=-1
    }
    \label{fig:ml_cycle}
    \vspace{-5mm}
\end{figure}



Reproducing an experiment (\Figref{fig:ml_cycle}(1)) can be done by obtaining the experiment object and evaluating it (e.g. calling its \TT{train} method). Since symbolic objects are serializable, users can obtain the experiment by loading it from a file or an experiment repository.
As we have discussed in \Secref{sec:symbolic-patching} extensively, iterating an experiment (\Figref{fig:ml_cycle}(3)) involves patching the experiment with pre-existing or new components. When new components are required, symbolic components can be created similarly as regular components plus applying a \TT{pg.symbolize} decorator (\Figref{fig:ml_cycle}(2)). Although an experiment can be manually iterated by hand, it is cumbersome to run all the experiments manually, especially when the combination of modifications results in a large space of experiments to explore. Symbolic placeholding makes automatic tuning (\Figref{fig:ml_cycle}(4)) easy - by replacing the values to tune with search space specifications, concrete experiments can be generated from the space under the control of tuning algorithms. Such tuning works for both hyperparameters and neural architectures, as well as other experiment parts such as losses, optimizers, data augmentation policies, and etc. Finally, when an experiment is ready for graduation (\Figref{fig:ml_cycle}(5)), it can be serialized into a file or saved in an experiment repository. Not only the experiment as a whole, but also its parts. New components and patching rules shall also be checked in as standard ML modules.

% If a new ML component is introduced, the component needs to be made available to the consumers of the experiment. This can be done by merging back the code to the right codebase based on the access level of the experiment.


% When the user start to evolve the experiment into new ones, developing new components are usually required. With {\NAME}, new ML components can be developed as a regular class with applying a . 


% n existing experiment, changing the combination or values of existing parts, or both.
% The mutability of symbolic object makes iterations straightforward: the user can (1) cherry-pick the experiment parts and change them, for example, applying the newly introduced \TT{MaskRCNN} model to a new dataset and modifying the learning rate; (2) apply rules to modify the experiment, for example, replacing all the \TT{ReLU} layers with the \TT{SquareReLU} layers; and (3) apply encapsulated techniques without knowing the implementation details, for example, the experiment can be patched with applying three techniques illustrated in \Figref{fig:ml_cycle}: scales up the batch size and learning rate simultaneously, applies the RMSProp optimizer and turns on AutoAugment~\cite{cubuk2019autoaugment}.

%\textbf{Automatic Tuning}
% Although an experiment can be manually iterated by hand, it is cumbersome to run all the experiments manually, especially when the combination of modifications results in a large space of experiments to explore.
% Symbolic placeholding makes automatic tuning easy - by replacing the nodes to tune with search space specifications, concrete experiments can be generated from the space by tuning algorithms. Such tuning works for both hyperparameters and neural architectures, as well as other experiment parts such as losses, optimizers, data augmentation policies, and etc.

%\textbf{Release}
% Finally, when an experiment is ready for graduation, it can be serialized into a file or saved in an experiment repository. If a new ML component is introduced, the component needs to be made available to the consumers of the experiment. This can be done by merging back the code to the right codebase based on the access level of the experiment.


%Experiment parts can be created as the objects of such symbolic classes, which are also serializable thus can be shared too. Besides, symbolic comparison, diff, and visualization can improve the developer tools substantially.



==> src/rebuttal/4_analysis.tex <==

\section{An Analysis of PyGlove's Approach}\label{sec:pyglove-analysis}


Behind the power of patching and the simplicity in how {\NAME} serves ML, there lies a more profound question - what is the essence of {\NAME}'s approach, and how does it compare with existing approaches in the context of ML?
We include a brief answer to this question as follows.\looseness=-1



{\NAME}'s approach to ML is focused on encapsulating the engineering efforts (e.g., modifying source code) that are involved in the journey from experiment A to experiment B. It is based on an insight that new ideas are much fewer than their applications and how they can be combined.
% Regarding developing components for new functionalities, {\NAME} does the same as the traditional approach.
PyGlove provides a unique solution for enabling flexible interfaces for ideas to be expressed, reused and shared easily.
More abstractly, {\NAME} enhances the object-oriented paradigm by adding symbolic programmability on objects, so the objects that represent ML experiments can be easily manipulated at run-time by rules, encapsulating the process of machine learning other than merely products.

\subsection{Comparison to Non-symbolic Solutions}

\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-15mm}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{src/figures/hp_container_v3.pdf}
  \end{center}
\vspace{-4mm}
\caption{
The separation of experiment representation (Left) and experiment definition (Right) in a non-symbolic ML program.
}
\vspace{-5mm}
\label{fig:hp_container}
\end{wrapfigure}
An apparent difference between {\NAME} and non-symbolic solutions lies in whether or not hyperparameter container is required to serve as a separate editable representation for a ML program, in contrast to experiment definition which are the ML components that implement the representation. In {\NAME}, an ML experiment (e.g., using Adam~\cite{kingma2015adam} to optimize a ResNet~\cite{he2016deep} model with cross-entropy loss) is represented as a symbolic object - a unity of experiment representation and definition.
While in non-symbolic solutions, since experiment definition is not directly mutable, it requires a separate editable representation as an indirection to create the experiment, illustrated in \Figref{fig:hp_container}.\looseness=-1

The separation of experiment representation and experiment definition not only causes redundancies but also introduces inconveniences due to a need for synchronization.
There are three common scenarios.
First, the developer needs to modify an component's representation when its paired definition is updated, and vice versa. Such synchronization includes but is not limited to documentation, validation rules, and logic for accommodating sub-component creations.
Second, when the user is working on an experiment representation, all automation tools that need to access its component definitions cannot simply work, such as auto-completion, code navigation, etc.
Third, when debugging a running experiment, to map the error back to the experiment representation is very difficult, especially when complex composition of the same component type is involved. For example, to identify which Conv layer has caused an input shape mismatch.

% The separation makes it difficult to encapsulate rules.
% When it comes to encapsulating rules, which is the main topic of this paper.
Encapsulating rules is difficult when the aforementioned separation exists.
This is because the separation of the two parties makes meta-programming difficult.
An example is to implement a \TT{change\_dataset} rule in \Figref{fig:symbolic_exp_complex_v1}-1.
We need to query the number of classes for that dataset, since the model head' width should be updated accordingly.
This was naturally implemented by invoking the \TT{num\_classes} property of the symbolic dataset object.
However, in a non-symbolic system, we will need to create a temporary dataset object from its representation to get the property.
% DXY: I just removed that, as I can not understand it easily.
% If this is still doable, then the following use case will be very difficult - a transformer model that requires a shared token embedder between the encoder and decoder network - this requires to break the 1:1 relationship between the definition and produced object, while through symbolic object, we can just pass the same object to two consumers.

\subsection{Caveats and Limitations}

{\NAME} employs a mutable programming paradigm, which comes with caveats and limitations.
By conventional wisdom, mutable programs are mainly criticized for three drawbacks.
(1) It is harder to program safely: since objects can change, it needs special care to ensure the program state is consistent upon mutations. (2) It is harder to reason about: downstream code may update objects created earlier; thus, it is more difficult to follow what is going on by simply looking at the code. (3) It is less performant: mutable objects need extra instructions for bookkeeping the arguments in order to handle mutation; thus, the creation of symbolic objects is slower than immutable objects. Moreover, using mutable objects for multi-threading is difficult due to the extensive locking required.
While the points are generally valid, we argue that we need to directly support it when mutability is necessary instead of being settled with a workaround.
In practice, we found that the real issues caused by mutability are rare when the program is designed properly, through extensive testing in applying {\NAME} to real-world use cases in both research and products. However, users should be informed about the run-time traits of symbolic objects.
Currently, each mutation on a tree with hundreds of sub-nodes takes only a sub-second, which might be fast enough for ML programs that train for hours or even days, but may significantly slow down programs whose evaluation takes milliseconds or less.

==> src/rebuttal/5_broader_impact.tex <==

\section{Broader Impact}\label{sec:limitation}

After providing a principled solution to AutoML~\cite{peng2020pyglove}, {\NAME} takes an essential step in tackling the issues in productivity and collaborations in ML, which, in our opinion, is critical for the sustainability of ML's advancement. With providing a solution for enabling network effect among ideas in ML, together with a guideline for scaling it up to multiple codebases, {\NAME} presents an ambitious vision for more collaborative ML, by maximizing the network effects among the entire ML community - Every member in the community can easy consume and contribute to other's work, not only experiments, but also rules. With reusable rules as higher-level description of experiments, the essential contributions of research publications can be communicated precisely and effortlessly; new discoveries can generalize better through more comprehensive studies and comparisons; and the adoption can happen much faster with much less cost. On the other end, a huge efficiency boost in ML engineering would significantly reduce the engineering need for ML by eliminating redundant efforts, which may lead to a decline in the demand for ML engineers.

==> src/submission/1_introduction.tex <==
\section{Introduction}\label{sec:introduction}

Thousands of machine learning (ML) papers are submitted each year to top-tier conferences and journals.
Many of these venues now encourage the open-sourcing of relevant code, such as NeurIPS or ICLR, highlighting the need for researchers and practitioners to share not only their ideas but also their implementation.
This is true within organizations too, which today can employ thousands. In particular, the training and deployment of large models now require multiple engineers and researchers to work together. Whether within a large group or the ML community as a whole, exchanging code to keep up with discoveries is essential.
For example, image classification has seen in recent years transitions from plain convolutional networks, to the introduction of batch normalization~\cite{ioffe2015batch}, residuals~\cite{he2016deep}, inverted bottlenecks~\cite{sandler2018mobilenetv2}, and a transition to transformers~\cite{vaswani2017attention}.
A team working on image classification that wants to keep their models up to date would have had to incorporate these changes either by adapting the external code through interfaces or simply rewriting it -- both time-consuming processes.
This is challenging because different teams develop their own conventions without any unifying standards. Our paper addresses this problem by extending {\NAME}~\cite{peng2020pyglove} to a language that allows defining flexible standards and writing rules for how to use the standards to exchange code easily.

Flexibility is key, as enforcing strict standards may limit long-term progress. This is because it can be difficult to avoid over-emphasizing our current ideas when defining conventions. For example, in 2015, we may have adopted an interface in which every layer receives only the activations of the previous layer, so in 2016 we would have had to rewrite our interface to include the skip-connections of a ResNet. Another example would have been to assume independence across examples at training time, which would need to be broken to apply batch-normalization. In each case, we made an assumption that was later broken by new discoveries. One possible solution is to simply accept that standards must evolve \cite{sussman2007building}. Thus, our approach allows defining editable standards.

To achieve these goals, {\NAME} takes a rule-based approach: standards are first defined by light-weight annotations of ML code and then rules indicate how the code should be shared. For example, consider a situation in which ``team A'' maintains an image classifier and ``team B'' independently comes up with a new convolutional layer that should improve most image classifiers. In the {\NAME} approach, team A can annotate their (pre-existing) code with statements akin to ``this is a convolution'', ``this is a nonlinearity'', and so on, and team B would annotate their new layer with statements akin to ``these are hyperparameters'' (see \Secref{sec:symbolic-patching}).
Up to this point in our example, the two teams need not have interacted at all. Upon team A learning about the new layer, A can write a one-line rule equivalent to ``replace all my convolutions with team B's layer'' (technically accurate examples in \Secref{sec:symbolic-patching}).
Additionally, {\NAME} also allows a novel twist: team B can write the replacement rule themselves -- such a rule would be analogous to ``in any image classifier, replace all convolutions with our layer''. Then any team with a {\NAME}-annotated image classifier can apply the rule produced by team B. This twist opens up future collaboration options through repositories of ML inventions, which we discuss in \Secref{subsec:patch-power}.

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-5mm}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{src/figures/network_effects_v3.pdf}
  \end{center}
  \label{fig:network-effects}
\vspace{-4mm}
\caption{
Applying $m$ new ML innovations to $n$ teams leads to $n{\times}m$ code changes.
{\NAME} expresses an ML innovation as a sharable rule that can be applied at once by each of the $m$ teams.
% Network effect among ML ideas: with existing ideas (expressed by rule -- a block), introducing a new idea can lead to an exponential growth of the applications of these ideas.
%
% A single additional patching rule (\#N+1) leads to 
%
%more than O(N) different kinds of experiments.
% 6 patching rules leads to 9 unique valid object detection experiments. Adding an experiment will double the number, creating a network effect.
}
\end{wrapfigure}
PyGlove's rule-based approach is not constrained to the sharing of architectural changes but applies to all aspects of the ML pipeline, such as data augmentation, training algorithm, or meta-learning. In particular, as ML hardware improves, there is a recurring need to scale up model capacity. Empirical and theoretical rules have been invented to address this problem~\cite{sussman2007building,tan2019efficientnet,yang2021tuning}. Such rules could be broadcasted throughout an organization or the community, saving valuable engineer time.
% Moreover, network effects are possible by combining these rules.
This is true even across codebases, provided the guidelines in \Secref{subsec:scale-ml-network-effect} are followed. \Figref{fig:network-effects} illustrates the efficiency gains through community network effects: without PyGlove $m$ innovations applied to $n$ team projects result in $m \times n$ work; with PyGlove, each innovation requires writing a PyGlove rule ($m$ rules) and each team project is responsible for PyGlove annotations in their own model ($n$ models), resulting in only $m + n$ work, as the rule application is trivial.
In addition to the sharing of code, {\NAME}'s rules can also allow an individual to manipulate their ML system. In all these cases, our rule-based approach stands in contrast to current methods, which typically require multiple in-place edits that do not scale well with the size of the model or with the number of practitioners in the community.
These comparisons are detailed in \Secref{sec:pyglove-analysis}.\looseness=-1



The reason why {\NAME} can be applied broadly to all aspects of ML code -- and indeed beyond ML -- is its principled symbolic programming design~\cite{mccarthy1960recursive}.
Under this paradigm, {\NAME}-annotated Python objects become editable symbols, and {\NAME} rules are meta-programs that act on these symbols.
The rules are also symbols themselves, allowing compositionality similar to that of a LISP program's ability to self-edit~\cite{steele1990common}.
In \Secref{sec:symbolic-program-ml}, we describe symbolic programming and explain the {\NAME} design.\looseness=-1

To summarize, our contributions are:
\begin{itemize}
    \item A novel annotation-based language to express flexible standards that can evolve over time;
    \item A principled, rule-based method for easily exchanging complex ML ideas as code;
    \item Guidelines for efficient {\NAME} usage across large teams or communities; and
    % \item a formalization of allowing programs to modify programs at runtime for ML.
    % \item a formalization of {\NAME}'s programming paradigm for ML
    \item A formulation of ML's life-cycle through a symbolic programming paradigm.
    % for machine learning.
    % \item a formalization of our method as symbolic programming for machine learning.
\end{itemize}

The final product, {\NAME}, is open-sourced with this paper.
%at GitHub \url{https://github.com/google/pyglove}.


==> src/submission/2_method.tex <==
\section{Expressing ML Ideas Through Patching }\label{sec:symbolic-patching}

The engineering process of ML is to journey from experiment A to experiment B, in which an iteration is made by manually applying the conceptual rules that formulate an idea to an ML program---a process of source code manipulation.
For example, supposing an ML practitioner wants to swap all the convolution layers with separable convolution layers in a neural network, the practitioner must locate the appearances of all convolution units in the model source code and replace each of them with the intended separable convolution.
To automate this process, we need the ML program to be manipulated programmatically. 
Such program modification is not only necessary to implement an idea but required to apply the same idea to other ML programs without complicating their codebases.
% A natural intuition is to allow an ML program to be dynamically modifiable at run time, which has been long offered by a symbolic programming paradigm originated from LISP~\cite{steele1990common}, later introduced to AutoML by {\NAME}\cite{peng2020pyglove}. Here we extend {\NAME}'s symbolic capacity from AutoML~\cite{peng2020pyglove} to ML, to express the rules embodied in the previous manual process and encapsulate them into reusable program units across different ML programs.
A natural intuition is to allow an ML program to be dynamically modifiable at run time. Motivated by this, we develop {\NAME} to express the rules embodied in the previous manual process and encapsulate them into reusable program units across different ML programs.
% ~\cite{hutchins1985direct}
As a result, not only a complex idea can be implemented by directly manipulating the ML programs, but also the laborious repetition of daily ML practices can be captured by such program expression of rules -- \emph{patches}.
The use case mentioned above in which team A applies team B's latest convolution invention without laborious manual coding is illustrated in \Figref{fig:symbolic_exp_sim_v1}.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\textwidth]{src/figures/patch_overview_v2.pdf}
    \includegraphics[width=0.9\textwidth]{src/figures/first_patch_simple_example_v4.pdf}
    \caption{
Team B's new invention \TT{SepConv} is developed agnostic to Team A's experiment, but its rule \TT{apply\_sepconv} can be patched to upgrade Team A's experiment into \TT{new\_resnet}.
In this code, \TT{pg.symbolize} is the annotation that adds the editable trait to regular Python classes, and \TT{pg.patch} is the operation that applies a rule to an object of an annotated class.
}
    \label{fig:symbolic_exp_sim_v1}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth]{src/figures/symbolic_exp_complex_v2.pdf}
    \caption{
Three more complex ideas are expressed via {\NAME} patching rules.
(Left) To change the dataset for a classification task, we need to change both the dataset and the model header's width to align with the number of classes.
This is done by querying the location of the last Dense layer, and returning the new value for both the dataset and the dense units associated with their locations as an update to the experiment.
(Middle) To multiply a scaling factor on the channels of the Conv and FC layer, the patching rule is defined by a function for transforming each node in the object tree, which takes the location, value and parent of current node as input, and modifies the `channels' member of Conv and FC classes. (Right) A upgraded version of previous example, which uses AutoML for scaling the model with a target FLOPs. To do so, it generates a search space of scale factors, and connects the search space to an AutoML trainer, which automatically figure out the best choices.
% based on the target flops.
}
    \label{fig:symbolic_exp_complex_v1}
\end{figure}






\subsection{The Power and Compositionality of Patching}   \label{subsec:patch-power}



\begin{wrapfigure}{r}{0.32\textwidth}
  \vspace{-6mm}
  \begin{center}
    \includegraphics[width=0.32\textwidth]{src/figures/patch_composition_v3.pdf}
  \end{center}
\vspace{-4mm}
\caption{
The LaMDA paper~\cite{thoppilan2022lamda} can be obtained by applying a composition of patches on the Transformer paper~\cite{wolf2020transformers}.
}
\vspace{-5mm}
\label{fig:patch_composition}
\end{wrapfigure}
The simplicity of {\NAME} to express rules is also applicable to more complex ideas.
With a capacity of direction manipulation~\cite{hutchins1985direct}, the user can modify program parts in an ML experiment by locations or by rules.
For example, \Figref{fig:symbolic_exp_complex_v1} illustrates how to change dataset, scale the width of neural models, and automatically scale the model by AutoML through {\NAME}.


% Patches themselves are symbolic objects \daiyip{Can we use it and refer to later section without definition?}(See \Secref{}), which can be serialized and moved across codebases and processes.

Simple patches can be combined together to express complex ideas.
For example, the recent large-scale NLP algorithm, LaMDA~\cite{thoppilan2022lamda}, can be obtained by applying common patches to the Transformer paper~\cite{wolf2020transformers}.
We briefly introduced how this can be implemented with {\NAME} in \Figref{fig:patch_composition}. 


Patches, i.e., program expression of rules, are useful not only because they make the expression of ideas straightforward but also because they can be shared freely and applied to different ML experiments.
{\NAME} allows patches themselves to be easily shared across codebases.
It allows users to create a patch from a URI-like string, which is human readable and can be easily referred to with a global unique name. For example, a patch for changing dataset to ImageNet~\cite{deng2009imagenet} can be described as \TT{``change\_dataset?name=imagenet''}.



% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-10mm}
%   \begin{center}
%     \includegraphics[width=0.45\textwidth]{xfigures/patch_network_effect_v1.pdf}
%   \end{center}
% \vspace{-4mm}
% \caption{
% 6 patching rules leads to 9 unique valid object detection experiments. Adding an experiment will double the number, creating a network effect.
% }
% \vspace{-1mm}
% \label{fig:patch_network_effect}
% \end{wrapfigure}


\begin{wrapfigure}{r}{0.58\textwidth}
  \vspace{-6mm}
  \begin{center}
    \includegraphics[width=0.58\textwidth]{src/figures/deep_network_effect_v4.pdf}
  \end{center}
\vspace{-4mm}
\caption{
Without {\NAME}, patching $m$ changes into $n$ teams requires $n\times{m}$ modifications to the code.
With {\NAME}, each $A_{i}$ team annotates their own code and each $B_{j}$ team writes their own rules.
As a result, patching all changes takes $n+m$ changes only.
}
\vspace{-8mm}
\label{fig:deep_network_effect}
\end{wrapfigure}
The compositionality of patches leads to a network effect among the ML ideas. We illustrate a common scenario in \Figref{fig:deep_network_effect}, that how research teams (Teams $B_{i}$) share their latest discoveries with product teams (Teams $A_{i}$). Based on {\NAME}, a research discovery can be encapsulated by a patching rule. Once the rule is created, any product team whose codebases are annotated by {\NAME} in a compatible way can apply it. This means that a research team's idea can be adopted by many product teams without manually integrating it each time. Similarly, a product team can try many research ideas quickly. This has not yet count the combination of patches, which can grow the degree of network effect exponentially. 


%\tododp{Revise the words to align with the new figures.}
% As illustrated in \Figref{fig:network-effects}, we have $3$ patching rules for data augmentation policies and $3$ patching rules for learning schedules.
% Then, we can get $3*3=9$ different experiments through combination, even if the learning schedules are mutually-exclusive and augmentation policies are also exclusive.
% Furthermore, when we add an experiment, for example, an image classification task, it will double the number of valid combinations. Therefore, once we have a fair amount of patching rules and experiments, the variety of valid experiments that can be expressed can grow exponentially.

% \tododxy{can you add a diagram here to illustrate the network effect described above?} # DONE

\subsection{Scaling Up the Network Effect of ML Ideas}\label{subsec:scale-ml-network-effect}

Patches need to be written wisely. For example, consider the following potential pitfall: assuming a research team has found a brilliant way to figure out the learning rate for image classifiers, they write a rule depending on a ``\TT{learning\_rate}'' property of the task after seeing it fit for an \TT{ImageClassificationTask} class.
Later someone in this team wants to apply the rule to another image classifier - \TT{ImgClsTask}, which, instead of having \TT{``learning\_rate''}, has a \TT{``lr''} property. The rule will surely fail due to the mismatch between the expected and actual locations for the learning rate. In such case, a better rule can be written as - matching any node under the task whose key is either \TT{``learning\_rate''} or \TT{``lr''}, which not only work for the cases above, but also for cases that specifies learning rate not as an immediate property of the task, but under its sub-node such as an optimizer.
This approach, however, does not scale well since the pre-defined assumptions cannot always meet the growth of heterogeneous components. As a result, to maximize the generality of rules, we need to reduce the discrepancies among ML components by advocating reuse at both the low level (e.g., network layers) and higher levels (e.g., training loop definition).

Standardization is the process of reducing the applicability issues for patching across codebases. It sounds alarming, as usually, standardization means reducing flexibility and autonomy.
In our proposal, however, we suggest an ML component ecosystem that carefully considers the flexibility and self-govern needs, while allowing different codebases to converge in what ML components they use incrementally. Such an ML ecosystem should have the following requirements:

\textbf{(1) Concept-oriented} Components in the ML ecosystem should precisely represent the concepts in the human mind. They should be able to be put together by composition and can be manipulated easily. ML components like this should allow a natural mapping of the concepts and straightforward expressions of ideas, which makes them competitive for broad adoption.


\textbf{(2) Scalable for extension} The components should be extensible without modifying the existing source code.
In other words, a component can be extended without modifying its class definition, and an object of the component should be able to be modified without changing its source code.

\textbf{(3) Runtime independence} The user-facing interfaces should be independent of the execution environment, such as ML frameworks, hardware accelerators, etc.
If so, it will allow the identical ML experiment definition to run consistently from everywhere.

\textbf{(4) Maximizing sharing} Both ML components and their objects can be easily shared. Moreover, ML objects of common interests, such as well-known experiments, can be retrieved with a globally unique identifier (e.g., URL), which automatically imports their required components.
Therefore, ML experiments and techniques can be easily referenced by their identifiers.

\textbf{(5) Adaptive to changes} The ML ecosystem needs to adapt to the rises and falls of standard components.
This requires a scalable way of upgrading the existing experiments with new components that replaces the old components.

\textbf{(6) Supporting accessibility} The advocate for sharing does not mean that everything needs to be public. Organizations or individuals are welcome to have their own assets, no matter it is IP reasons or certain assets are too early to be shared publicly. Accessibility can be controlled at both component level and object level.

{\NAME} provides solutions to all these requirements:
\begin{itemize}
    \item A PyGlove-annotated object is a straightforward solution for developing concept-oriented components, which is compositional and mutable, addressing requirement (1).
    \item A PyGlove-annotated class can be extended by subclassing, and its object can be modified with manipulation, satisfying requirement (2).
    \item Patches can be easily developed to map common PyGlove-annotated classes to their runtime-specifc versions. Therefore, the user-facing components are decoupled completely from the components for implementation, meeting requirement (3).
    \item PyGlove-annotated objects are serializable, which can be stored in a file or database. Moreover, the serialized information contains the information for importing their components, so users can load the object through a single URL, addressing requirement (4).
    \item Upgrading an old component in existing experiments can be described as a patch, which can be triggered periodically on existing experiments, meeting requirement (5).
    \item Requirement (6) can be achieved easily with existing source control solutions.
\end{itemize}

%
% \tododxy{can you please insert a figure for supporting runtime independence?}
%\subsection{An Ultimate Goal}


% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-7mm}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{xfigures/final_picture_v1.pdf}
%   \end{center}
% \vspace{-3mm}
% \caption{
% The experiment of the LaMDA\cite{} paper can be be described as a previous experiment combined with existing or new techniques.
% }
% \vspace{-6mm}
% \label{fig:final_picture}
% \end{wrapfigure}



==> src/submission/3_symbolic_ml.tex <==


\section{Symbolic Programming for Machine Learning}\label{sec:symbolic-program-ml}


Patching demonstrates a unique angle to view machine learning programs through a lens of symbols, which directly maps the concepts from the human mind to computer program expressions~\cite{sussman2007building}. Symbolic programming, however, has a much broader usage in the entire life-cycle of ML than just patching. Before we get to that point, let's take a brief look at what symbolic programming is, why we need it in ML, and what's PyGlove's offering about it.

Symbolic programming, which originated from \cite{steele1990common}, is a programming paradigm to manipulate its own components as if they were plain data~\cite{mccarthy1960recursive}.
Symbolic programming is interesting to ML since ML is overloaded with a constant need for modifying the source code of  ML programs.
It accommodates the ideas that can not be done with predefined interfaces and frequently changed hyperparameters. When rules are introduced to change the behavior of programs, they either need to change the source code or manipulate them at run time. The former is not viable for ML, since ML requires different experiments to be obtained from the same source code. The other option seems to be a more flexible solution to try. Have we considered code generation?
Of course, manipulation has to be done with code generation at run time. But what about generating source code?
Our answer is no.
It is neither easy nor flexible, because (1) it requires templates for the source code, which are not generally applicable to all existing code, and (2) it is difficult to accommodate complex manipulation patterns, such as mutate-run-mutate, which is commonly needed in ML. For example, in \Figref{fig:symbolic_exp_complex_v1}-1, to change the dataset for an ML classifier, we need to generate code for loading that dataset by a name, evaluate it to get the number of classes for the task, and then apply the number to generate the code of the model head width.


\subsection{PyGlove's Symbolic Programming Solution}


PyGlove formulates its symbolic programming solution through the concept of symbolic object.
A symbolic object is a unity of symbol and object, with the two aspects synchronized, meaning that \textit{a symbolic object can be manipulated as a symbol, while it can be evaluated as a regular object}.
A symbolic object is an instance of a symbolic class, which can be created by annotation \TT{pg.symbolize}, illustrated in \Figref{fig:symbolic_ops}(1). While the class can be used as a regular class, this tiny decorator makes the operations illustrated in \Figref{fig:symbolic_ops}(2-8) applicable to its objects. Symbolic object has many characteristics: first of all, the construction information (type, constructor arguments) is preserved, which defines its \emph{symbolic representation}. Such representation is identical between its source form and run-time form, thus carries necessary information to fully embody the concept that the object represents. As a result, such representation is a proxy to the concept for manipulations - ideas can be expressed as direct manipulation~\cite{hutchins1985direct} of concepts through their symbolic representations. On the other hand, a symbolic object is also a program entity that exists at run time, which carries data members and methods, behaving like a regular object. The unity of being symbolic and being an object allows a symbolic object to take advantage of the capabilities from both object-oriented programming and symbolic programming, while the former allows a modular and extensible software design, the latter brings the power of meta-programming through manipulations.


\begin{figure}[h!]
    %\vspace{-5mm}
    \centering
    \includegraphics[width=0.90\textwidth]{src/figures/ml_symboy_ops_v1.pdf}
    \caption{The definition of a symbolic class, its instance (an symbolic object), and common symbolic operations that can be applied on it. A symbolic object can be developed, validated, inspected, compared, cloned, serialized, mutated, place-held and generated with ease.}
    \label{fig:symbolic_ops}
    \vspace{-1mm}
\end{figure}



\subsection{How Symbolic Object Serves Machine Learning End-to-End}


%Now we take a breadth-first view at how PyGlove serves the life-cycle of ML. \Figref{fig:symbolic_ops} shows the symbolic operations that are used during daily ML workflows. Through \Figref{fig:ml_cycle}, we demonstrate the combination of such operations can effectively address the requirements from different phases of the ML life-cycle, from reproduction to release.

Let us take a closer look at how symbolic object serves ML.
First, the mutability of symbolic object removes the need for hyperparameter containers, which makes the development and use of ML components much simpler and more consistent. Second, the combination of symbolic operations can effectively address the need of ML experimentation with a few lines of code. \Figref{fig:ml_cycle} illustrates the symbolic operations involved in the ML life-cycle based on the \TT{MLExperiment} class defined in \Figref{fig:symbolic_ops}.\looseness=-1




\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{src/figures/ml_experiment_cycle_v4.pdf}
    \caption{
    {\NAME} serves the ML life-cycle.
    {\NAME} simplifies the engineering efforts involved from the birth of a research idea to its graduation while making the whole or parts of an experiment reusable.\looseness=-1
    }
    \label{fig:ml_cycle}
    \vspace{-5mm}
\end{figure}



Reproducing an experiment (\Figref{fig:ml_cycle}(1)) can be done by obtaining the experiment object and evaluating it (e.g. calling its \TT{train} method). Since symbolic objects are serializable, users can obtain the experiment by loading it from a file or an experiment repository.
As we have discussed in \Secref{sec:symbolic-patching} extensively, iterating an experiment (\Figref{fig:ml_cycle}(3)) involves patching the experiment with pre-existing or new components. When new components are required, symbolic components can be created similarly as regular components plus applying a \TT{pg.symbolize} decorator (\Figref{fig:ml_cycle}(2)). Although an experiment can be manually iterated by hand, it is cumbersome to run all the experiments manually, especially when the combination of modifications results in a large space of experiments to explore. Symbolic placeholding makes automatic tuning (\Figref{fig:ml_cycle}(4)) easy - by replacing the values to tune with search space specifications, concrete experiments can be generated from the space under the control of tuning algorithms. Such tuning works for both hyperparameters and neural architectures, as well as other experiment parts such as losses, optimizers, data augmentation policies, and etc. Finally, when an experiment is ready for graduation (\Figref{fig:ml_cycle}(5)), it can be serialized into a file or saved in an experiment repository. Not only the experiment as a whole, but also its parts. New components and patching rules shall also be checked in as standard ML modules.

% If a new ML component is introduced, the component needs to be made available to the consumers of the experiment. This can be done by merging back the code to the right codebase based on the access level of the experiment.


% When the user start to evolve the experiment into new ones, developing new components are usually required. With {\NAME}, new ML components can be developed as a regular class with applying a . 


% n existing experiment, changing the combination or values of existing parts, or both.
% The mutability of symbolic object makes iterations straightforward: the user can (1) cherry-pick the experiment parts and change them, for example, applying the newly introduced \TT{MaskRCNN} model to a new dataset and modifying the learning rate; (2) apply rules to modify the experiment, for example, replacing all the \TT{ReLU} layers with the \TT{SquareReLU} layers; and (3) apply encapsulated techniques without knowing the implementation details, for example, the experiment can be patched with applying three techniques illustrated in \Figref{fig:ml_cycle}: scales up the batch size and learning rate simultaneously, applies the RMSProp optimizer and turns on AutoAugment~\cite{cubuk2019autoaugment}.

%\textbf{Automatic Tuning}
% Although an experiment can be manually iterated by hand, it is cumbersome to run all the experiments manually, especially when the combination of modifications results in a large space of experiments to explore.
% Symbolic placeholding makes automatic tuning easy - by replacing the nodes to tune with search space specifications, concrete experiments can be generated from the space by tuning algorithms. Such tuning works for both hyperparameters and neural architectures, as well as other experiment parts such as losses, optimizers, data augmentation policies, and etc.

%\textbf{Release}
% Finally, when an experiment is ready for graduation, it can be serialized into a file or saved in an experiment repository. If a new ML component is introduced, the component needs to be made available to the consumers of the experiment. This can be done by merging back the code to the right codebase based on the access level of the experiment.


%Experiment parts can be created as the objects of such symbolic classes, which are also serializable thus can be shared too. Besides, symbolic comparison, diff, and visualization can improve the developer tools substantially.



==> src/submission/4_analysis.tex <==

\section{An Analysis of PyGlove's Approach}\label{sec:pyglove-analysis}


Behind the power of patching and the simplicity in how {\NAME} serves ML, there lies a more profound question - what is the essence of {\NAME}'s approach, and how does it compare with existing approaches in the context of ML?
We include a brief answer to this question as follows.\looseness=-1



{\NAME}'s approach to ML is focused on encapsulating the engineering efforts (e.g., modifying source code) that are involved in the journey from experiment A to experiment B. It is based on an insight that new ideas are much fewer than their applications and how they can be combined.
% Regarding developing components for new functionalities, {\NAME} does the same as the traditional approach.
PyGlove provides a unique solution for enabling flexible interfaces for ideas to be expressed, reused and shared easily.
More abstractly, {\NAME} enhances the object-oriented paradigm by adding symbolic programmability on objects, so the objects that represent ML experiments can be easily manipulated at run-time by rules, encapsulating the process of machine learning other than merely products.

\subsection{Comparison to Non-symbolic Solutions}

\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-15mm}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{src/figures/hp_container_v3.pdf}
  \end{center}
\vspace{-4mm}
\caption{
The separation of experiment representation (Left) and experiment definition (Right) in a non-symbolic ML program.
}
\vspace{-5mm}
\label{fig:hp_container}
\end{wrapfigure}
An apparent difference between {\NAME} and non-symbolic solutions lies in whether or not hyperparameter container is required to serve as a separate editable representation for a ML program, in contrast to experiment definition which are the ML components that implement the representation. In {\NAME}, an ML experiment (e.g., using Adam~\cite{kingma2015adam} to optimize a ResNet~\cite{he2016deep} model with cross-entropy loss) is represented as a symbolic object - a unity of experiment representation and definition.
While in non-symbolic solutions, since experiment definition is not directly mutable, it requires a separate editable representation as an indirection to create the experiment, illustrated in \Figref{fig:hp_container}.\looseness=-1

The separation of experiment representation and experiment definition not only causes redundancies but also introduces inconveniences due to a need for synchronization.
There are three common scenarios.
First, the developer needs to modify an component's representation when its paired definition is updated, and vice versa. Such synchronization includes but is not limited to documentation, validation rules, and logic for accommodating sub-component creations.
Second, when the user is working on an experiment representation, all automation tools that need to access its component definitions cannot simply work, such as auto-completion, code navigation, etc.
Third, when debugging a running experiment, to map the error back to the experiment representation is very difficult, especially when complex composition of the same component type is involved. For example, to identify which Conv layer has caused an input shape mismatch.

% The separation makes it difficult to encapsulate rules.
% When it comes to encapsulating rules, which is the main topic of this paper.
Encapsulating rules is difficult when the aforementioned separation exists.
This is because the separation of the two parties makes meta-programming difficult.
An example is to implement a \TT{change\_dataset} rule in \Figref{fig:symbolic_exp_complex_v1}-1.
We need to query the number of classes for that dataset, since the model head' width should be updated accordingly.
This was naturally implemented by invoking the \TT{num\_classes} property of the symbolic dataset object.
However, in a non-symbolic system, we will need to create a temporary dataset object from its representation to get the property.
% DXY: I just removed that, as I can not understand it easily.
% If this is still doable, then the following use case will be very difficult - a transformer model that requires a shared token embedder between the encoder and decoder network - this requires to break the 1:1 relationship between the definition and produced object, while through symbolic object, we can just pass the same object to two consumers.

\subsection{Caveats and Limitations}

{\NAME} employs a mutable programming paradigm, which comes with caveats and limitations.
By conventional wisdom, mutable programs are mainly criticized for three drawbacks.
(1) It is harder to program safely: since objects can change, it needs special care to ensure the program state is consistent upon mutations. (2) It is harder to reason about: downstream code may update objects created earlier; thus, it is more difficult to follow what is going on by simply looking at the code. (3) It is less performant: mutable objects need extra instructions for bookkeeping the arguments in order to handle mutation; thus, the creation of symbolic objects is slower than immutable objects. Moreover, using mutable objects for multi-threading is difficult due to the extensive locking required.
While the points are generally valid, we argue that we need to directly support it when mutability is necessary instead of being settled with a workaround.
In practice, we found that the real issues caused by mutability are rare when the program is designed properly, through extensive testing in applying {\NAME} to real-world use cases in both research and products. However, users should be informed about the run-time traits of symbolic objects.
Currently, each mutation on a tree with hundreds of sub-nodes takes only a sub-second, which might be fast enough for ML programs that train for hours or even days, but may significantly slow down programs whose evaluation takes milliseconds or less.

==> src/submission/5_broader_impact.tex <==

\section{Broader Impact}\label{sec:limitation}

After providing a principled solution to AutoML~\cite{peng2020pyglove}, {\NAME} takes an essential step in tackling the issues in productivity and collaborations in ML, which, in our opinion, is critical for the sustainability of ML's advancement. With providing a solution for enabling network effect among ideas in ML, together with a guideline for scaling it up to multiple codebases, {\NAME} presents an ambitious vision for enabling 10x-100x faster development of ML, by maximizing the network effects among the entire ML community - Every member in the community can easy consume and contribute to other's work, not only experiments, but also rules. With reusable rules as higher-level description of experiments, the essential contributions of research publications can be communicated precisely and effortlessly; new discoveries can generalize better through more comprehensive studies and comparisons; and the adoption can happen much faster with much less cost. On the other end, a huge efficiency boost in ML engineering would significantly reduce the engineering need for ML by eliminating redundant efforts, which may lead to a decline in the demand for ML engineers.

==> src/submission/6_related_work.tex <==

\section{Related Work}\label{sec:related-work}



PyGlove joins the many software libraries for ML~\cite{abadi2016tensorflow,jax2018github,paszke2019pytorch, bergstra2010theano,jia2014caffe,chen2015mxnet,wu2019detectron2, tensorflowmodelgarden2020,shen2019lingvo}, but it is the first among its kind.
Instead of adding concrete features to ML programs, it introduces a novel programming paradigm for ML by obtaining an experiment from another experiment by applying rules. As a result, not only the ideas in ML can be expressed more easily with the rules, but also can the rules be reused, shared, and combined to make a network effect among the ideas collectively.
{\NAME}'s formulation of ML engineering process is similar to the transform pipelines in compilers~\cite{bacon1994compiler, lattner2004llvm}, which take the intermediate representation (IR) of programs as input and apply transforms on top of it in chains.
The IR in {\NAME} is the symbolic representation of the object, and the transforms are the patching rules. Though similar in how they frame the problem, there are a few noticeable differences: (1) In {\NAME}, the rules are applied on the program itself, while for compilers, the transforms are applied on other programs' IR. (2) The unity of IR and execution in {\NAME} allows the modification and execution of a program to mix, which enables more dynamic run-time behaviors.\looseness=-1

{\NAME}'s solution is a type of symbolic programming~\cite{mccarthy1960recursive}. However, different from most symbolic programming solutions, such as is in LISP~\cite{steele1990common}, in which manipulations are usually done at the code definition level, {\NAME}'s solution - symbolic object - enables manipulations at the object level. As a result, it's more powerful in that it allows the same code definition to have multiple instances that can be manipulated. Also, the manipulation is safer since it operates on the binding parameters of an object, instead of the lower-level code implementations, which are usually self-sufficient. To be precise, {\NAME}'s symbolic paradigm is a mixture of symbolic programming and object-oriented programming~\cite{stefik1985object} (OOP). It allows a symbolic object to be manipulated as a symbol and evaluated as an object. Therefore, it can take advantage of the benefits of both programming paradigms - while the former allows manipulation of programs, the latter allows developing reusable components by applying the best practices of OOP through encapsulation and inheritance.\looseness=-1

Within the ML community, the most relevant work on applying symbolic programming to ML is \cite{peng2020pyglove}, which reformulates the AutoML as a process of algorithm-based symbolic manipulations. It can be viewed as a specialized application of {\NAME} in the field of ML. To extend its applicability to the broader ML, we formalize the symbolic object paradigm, emphasize the encapsulation of rules, and the network effect among them. Therefore, this paper is not a simple repetition of previous work, but an extension and generalization.\looseness=-1


% One major reason behind the rapid growth of ML in the last decade is the productivity provided by different ML libraries.
% Back to the early 2000s, researchers have to write the back-propagation for each layer in C, CUDA, or MATLAB.
% Later, Theano~\cite{bergstra2010theano}, Caffe~\cite{jia2014caffe}, MXNet~\cite{chen2015mxnet} are developed that ML practitioners can explore ideas and deploy easier.
% Following them, TensorFlow~\cite{abadi2016tensorflow}, PyTorch~\cite{paszke2019pytorch}, and JAX~\cite{jax2018github} further push the productivity for ML practitioners.
% These libraries provided basic low-level ML components, such convolution layer or optimizer.
% Upon these libraries, thousands of algorithm codebases are built to encapsulate the entire ML algorithms, such as Detectron2~\cite{wu2019detectron2} and Lingvo~\cite{shen2019lingvo}.
% Until then, exploring a new idea on an ML algorithm usually means to modify the algorithm source code.
% Such paradigm is not scalable, if you want to try it on hundreds different algorithms or ship it to tens of products.
% {\NAME} provided a principled solution to encapsulate rules (idea) and easily exchange and apply it everywhere.
% As a result, plugging {\NAME} into these the existing ML libraries/codebases can further boost the productivity to the next scale -- ultimately scaling the network effect in ML.



% The capability of {\NAME} mainly came from converting class and function into the symbolic object.
% Within the ML community, the most relevant work is \cite{peng2020pyglove}, which uses symbolic programming to program and reformulate AutoML algorithms. It can be viewed as a specialized application of {\NAME} in the field of AutoML. To extend its applicability to the broader ML, we propose to build an arbitrary ML program based on the concept of symbolic object. Therefore, this paper is not a simple repeat of previous method, but a generalization and a formalization of the symbolic paradigm.


% Symbolic object takes root in object-oriented programming and symbolic programming.
% Object-oriented programming refers to a programming paradigm based on the concept of ``objects'', which can contain data and code~\cite{stefik1985object}.
% Symbolic programming is a programming paradigm in which the program can manipulate its own formulas and program components as if they were plain data~\cite{mccarthy1960recursive}.
% The core of {\NAME} - symbolic object - benefits from both symbolic programming and object-oriented programming.
% Instead of using separate and independent entities as symbols in symbolic programming, we equip regular objects with symbolic programmability. Therefore, objects can also work as symbols, with the two aspects always synchronized during manipulations.

==> src/submission/backup/2_method_2022_0518_0901.tex <==
\section{Symbolic Patches: Encapsulating Rules}\label{sec:symbolic-ml}

The engineering process of ML is to get from experiment A to experiment B, in which an iteration is made by manually applying the conceptual rules that formulate an idea to an ML program - a process of manipulating its source code.
For example, suppose an ML practitioner wants to swap all the convolution layers with separable convolution layers in a neural network.
This practitioner must locate all the convolution appearances in the model source code and replace everyone with an intended separable convolution.
To automate this process, we need the ML program to be manipulated by programs as if its source code is modified. 
Such logical program modification is not only necessary to implement an idea but required to apply the same idea to other ML programs without messing up with their codebases.
A natural intuitive solution is to allow an ML program to be dynamically modifiable at run time, which has been long offered by a symbolic programming paradigm originated from LISP~\dxy{cite}, later introduced to AutoML by {\NAME}\cite{peng2020pyglove}. Here we extend {\NAME}'s symbolic capacity from AutoML~\cite{peng2020pyglove} to ML, to express the conceptual rules embodied in the previous manual process and encapsulate them to make them reusable across different ML programs.
As a result, the laborious repetition of daily ML practices can be captured by such program expression of rules -- patches.
The story mentioned above in which team A applies team B's latest convolution invention without laborious manual translation has been be illustrated in \Figref{fig:symbolic_exp_sim_v1}.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{sfigures/symbolic_example_simplified_v2.pdf}
    \caption{
Team B's new invention \TT{SepConv} is developed agnostic to Team A's experiment, but its rule \TT{apply\_sepconv} can be patched to upgrade Team A's experiment into \TT{new\_resnet}.
In this code, \TT{pg.symbolize} is the annotation that adds the editable trait to regular Python classes, and \TT{pg.patch} is the operation that applies a rule to an object of an annotated class.}
    \label{fig:symbolic_exp_sim_v1}
\end{figure}



\begin{figure}[b!]
    \centering
    \includegraphics[width=\textwidth]{sfigures/symbolic_exp_complex_v1.pdf}
    \caption{
Three more complex ideas are easily expressed via {\NAME}.
(Left) To change the dataset for a classification task, we need to change both the dataset and the model header's width to align with the number of classes.
This is done by querying the location of the last Dense layer, and returning the new value for both the dataset and the dense units associated with their locations as an update to the experiment.
(Middle) To multiply a scaling factor on the channels of the Conv and FC layer, the patching rule is defined by a function for transforming each node in the object tree, which takes the location, value and parent of current node as input, and identifies the `channels' member of Conv and FC classes. (Right). 
}
    \label{fig:symbolic_exp_complex_v1}
\end{figure}





\paragraph{Expression Power}
The simplicity of {\NAME} to express rules is also applicable to more complex ideas.
With a capacity of direction manipulation~\dxy{cite}, the user can modify program parts in an ML experiment by locations or by rules.
For example, \Figref{fig:symbolic_exp_complex_v1} illustrates how to change dataset, scale the width of neural models, and automatically scale the model by AutoML via {\NAME}.


\paragraph{Re-usability}
Patches are useful not only because they make the expression of ideas straightforward but also because they can be shared freely and applied to different ML experiments.
% Patches themselves are symbolic objects \daiyip{Can we use it and refer to later section without definition?}(See \Secref{}), which can be serialized and moved across codebases and processes.
{\NAME} allows patches themselves to be serialized and moved across codebases.
Moreover, {\NAME} allows users to create a patch from a URI-like string, which is human readable and can be easily referred to with a global unique name. For example, a patch for changing dataset to ImageNet~\cite{deng2009imagenet} can be described as \TT{``change\_dataset?name=imagenet''}.



\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-4mm}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{sfigures/symbolic_exp_coms_lambda_v2.pdf}
  \end{center}
\vspace{-4mm}
\caption{
Placehold
}
\vspace{-5mm}
\label{fig:patch_composition}
\end{wrapfigure}
\paragraph{Compositionality}
Simpler patches can be combined together to express complex ideas.
For example, the recent large-scale NLP algorithm, LaMDA~\cite{thoppilan2022lamda}, can be obtained by applying common patches to the Transformer paper~\cite{wolf2020transformers}.
We briefly introduced how this can be implemented with {\NAME} in \Figref{fig:patch_composition}. 




\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-4mm}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{xfigures/patch_network_effect_v1.pdf}
  \end{center}
\vspace{-4mm}
\caption{
6 patching rules leads to 9 unique valid object detection experiments. Adding an experiment we can double the number, creating a network effect.
}
\vspace{-1mm}
\label{fig:patch_network_effect}
\end{wrapfigure}

\paragraph{Network Effect}
The compositionality of patches leads to a network effect: 
For example, we have $3$ patching rules for data augmentation policies and $3$ patching rules for learning schedules.
Then, we can get $3*3=9$ different experiments through combination, even if the learning schedules are mutually-exclusive and augmentation policies are also exclusive.
Furthermore, when we add an experiment, for example, an image classification task, it will double the number of valid combinations. Therefore, once we have a fair amount of patching rules and experiments, the variety of valid experiments that can be expressed can grow exponentially.




==> src/submission/backup/3_scaleup_2022_0518_1020.tex <==

\section{Scaling Up Network Effect}\label{sec:scale-ml-network-effect}

\subsection{Applicability of Symbolic Patches}

%More than that, the implementation of a patch also limit its applicability. For example, 
A symbolic patch is a (meta-)program that operates on ML programs based on certain assumptions.
Its applicability to different experiments depends on whether its assumptions generalize well. 
The assumptions have to be programmed against its input, which are 1) the location; 2) the value along with its type; and 3) the parent node of the current node that is being worked in the symbolic tree (See \Secref{sec:how-pyglove-works}). 
%in a single codebase or across heterogeneous codebases 
The location dependencies are weaker comparing to the type or value dependencies, because it relies on a more restrictive pattern recognition rule by identifying a node in a fixed topology. This can easily get broken when the patches are applied across codebases, due to the fact that different codebase usually have heterogeneous high-level ML components which maintain a different composition hierarchy. To minimize such risks, we need to advocate more reuse on both low-level (e.g. network layers) and higher-level (e.g. training loop definition) ML components. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{xfigures/patch_applicability_v1.pdf}
    \caption{
 A conceptually same experiment expressed in different ways leads to applicability issues for \TT{change\_lr}, but does not hinder \TT{swap\_relu} since it's based on more robust pattern recognition rules.
}
    \label{fig:patch_applicability}
\end{figure}


%less general because heterogeneous codebases may have very different descriptions for a conceptually similar experiment.
%The type and value dependencies can be more general when common ML component are used in different experiments. However, when across ML codebases, these dependencies may also facing difficulties \dxy{examples}.
%Oftentimes, the assumptions would break in practice, which is more often when patches are applied across codebases than under a single codebase, due to the fact that different codebases usually have heterogeneous representations of a similar experiment




\subsection{Standardizing ML Components for Network Effects}\label{subsec:requirement-network-effect}

Standardizing is a process for reducing the applicability issues for patching across codebases. It sounds scary, as usually standardization means to reduce flexibility and autonomy. In our proposal, however, we suggest a ML system that carefully 
consider the flexibility and self-govern need, while allows different codebases to converge in ML components they use, in an incremental way. Such ML system should have the following traits:

%To make patching rules more general across codebases, we need to advocate the reuse of ML components through a standardization process.
%To be open to extending and optimizing for reuse, the ecosystem of components should meet the following requirements.


\textbf{(1) Concept-oriented} Components in the ML system should precisely represent the concepts in the human mind. They should be able to be put together by composition and can be manipulated easily. ML components like this should allow a natural mapping of the concepts and straightforward expressions of ideas, which makes them competitive for broad adoption.

\textbf{(2) Scalable for extension} The components should be extensible without modifying existing source code. This means (1) a component can be extended without modifying its class definition, and (2) an object of the component should be able to be modified without changing its source code.

\textbf{(3) Runtime independent} The user-facing interfaces should be independent from the execution environment, such as ML frameworks, hardware accelerators, etc.
If so, it will allow the same ML experiment definition to run consistently from everywhere.

\textbf{(4) Maximizing sharing} Both ML components and their objects can be easily shared. Moreover, ML objects of common interests, such as well-known experiments, can be retrieved with a globally unique identifier (e.g. URL), which automatically imports their required components.
Therefore, ML experiments and techniques can be easily referenced by their identifiers.

\textbf{(5) Adaptive to changes} The ML system needs to adapt to the rises and falls of standard components.
This requires a scalable way of upgrading the existing experiments with new components that replaces the old components.

\textbf{(6) Supporting accessibility} The advocate for sharing does not mean that everything needs to be public. Organizations or individuals are welcome to have their own assets, no matter it be IP reasons or certain assets are too early to be shared publicly. Accessibility can be controlled at both component lvel and object level.


\subsection{{\NAME}'s Solution}\label{subsec:pg-solution-scale-network-effect}

{\NAME} provides unique solutions to address requirements (1) - (5):
\begin{itemize}
    \item A PyGlove-annotated object is a straightforward solution for developing concept-oriented components, which is compositional and mutable, addressing requirement (1). 
    \item A PyGlove-annotated class can be extended by subclassing, and its object can be modified with manipulation, satisfying requirement (2).
    \item Patches can be easily developed to map common PyGlove-annotated classes to their runtime-specifc versions. Therefore, the user-facing components are decoupled completely from the components for implementation, meeting requirement (3).
    \item PyGlove-annotated objects are serializable, which can be stored in a file or database. Moreover, the serialized information contains the information for importing their components, so users can load the object through a single URL, addressing requirement (4).
    \item Upgrading an old component in existing experiments can be described as a patch, which can be triggered periodically on existing experiments, meeting requirement (5).
    
\end{itemize}

\daiyip{Consider to insert examples if space allows}
Requirement (6) can be done easily with existing source control solutions.

%\subsection{An Ultimate Goal}


% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-7mm}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{xfigures/final_picture_v1.pdf}
%   \end{center}
% \vspace{-3mm}
% \caption{
% The experiment of the LaMDA\cite{} paper can be be described as a previous experiment combined with existing or new techniques.
% }
% \vspace{-6mm}
% \label{fig:final_picture}
% \end{wrapfigure}



==> src/submission/backup/7_conclusion.tex <==
\section{Conclusion}

Machine learning is bottle-necked by the inability of applying conceptual rules to different experiments in a scalable way. Even when the code for a publication is open sourced, its experiment definition is shared, the process for obtaining that experiment from a regular experiment is neither obvious nor reusable. It has to be parsed by human and replicated on other experiments manually. In this paper, we have extended PyGlove~\cite{peng2020pyglove}'s symbolic capabilities from AutoML to ML, to solve this problem. In our proposal, the process for evolving an experiment A to experiment B is decomposed into a list of patching rules, which can be reused across experiments - even codebases, resulting network effects among the experiments and such rules. We further discussed how to scale up such network effect by building a principled ML component ecosystem based on PyGlove, demonstrated how the symbolic approach serves ML well. We also compared PyGlove's solution with non-symbolic solutions. Through real-world research projects that extensively depend on PyGlove's patching capability~\cite{dong2021autohas,zhou2022towards}, we have seen a prospect in how PyGlove can change the ways in which ML programs are developed, organized and shared. We open-source PyGlove and look forward to its symbolic power to be thoroughly tested and used by the machine learning community.

%\tododp{rewrite this section}

% The rapid development of ML has led to fragmented ML codebases, which become an increasing bottleneck for ML to scale.
% In this paper, we analyze the obstacles for these codebases to be more collaborative: we attribute the difficulties of reusing code largely to the presence of hyperparameter containers, which in turn causes the proliferation of high-level interfaces for ML.
% To overcome these obstacles, we propose a symbolic approach for developing ML programs, which removes the need for hyperparameter containers and better serves the need for ML with simplicity and flexibility.
% We further discuss a path to converge the fragmented high-level ML interfaces, through an analysis of its requirements, ingredients, and potential outcomes.
% We believe that we are better equipped than ever to break the barriers of reusing code in ML.
% Therefore, we appeal to everyone in the ML community that by working closely together, we can make the future of machine learning more collective.

==> src/submission/backup/abstract.tex <==
\begin{abstract}
The recent growth in the scale of machine learning (ML) has resulted in large groups involving tens — or thousands — of researchers and engineers. Sub-teams must work independently but they must also exchange code efficiently. This exchange, however, is strongly limited by the lack of standards for how different aspects of ML interact (model components, training algorithms, hyperparameter containers). For example, if team A invents a new type of convolutional layer, team B should be able to reuse it with minimal additional code. On the other hand, strict standards can impede research due to its paradigm-breaking nature. In our example, if team B were to define a strict interface for standard convolutional layers, it may face difficulties transitioning to a ResNet-like architecture with skip-connections. Therefore, we would like to have flexible, efficiency-oriented standards that evolve as the field progresses.
In this paper, we extend PyGlove~\cite{peng2020pyglove} to achieve this goal and open-source it.
% In this paper, we extend PyGlove to achieve this goal, and we open-source it \footnote{https://github.com/google/pyglove}.
PyGlove is a lightweight library that can annotate Python code to define an editable standard for how components should interact. Its rule-based approach then allows quickly incorporating new ideas into a codebase for fast iteration. For example, it makes it possible with one line of code to insert skip-connections everywhere. Moreover, it provides a language for sharing those rules allowing the inventors themselves to write down the rules for models they have not seen. Behind the scenes, PyGlove generates all the necessary interfacing code in a principled manner using a symbolic programming paradigm.
This paper describes this symbolic PyGlove design, demonstrates its practical use in ML through comparisons to existing approaches, and speculates about a potential path toward productive ML collaboration at the next scale.
\end{abstract}


==> src/submission/backup/submission/1_introduction.tex <==
\section{Introduction}\label{sec:introduction}

Thousands of machine learning (ML) papers are submitted each year to top-tier conferences and journals.
Many of these venues now encourage the open-sourcing of relevant code, such as NeurIPS or ICLR, highlighting the need for researchers and practitioners to share not only their ideas but also their implementation.
This is true within organizations too, which today can employ thousands. In particular, the training and deployment of large models now require multiple engineers and researchers to work together. Whether within a large group or the ML community as a whole, exchanging code to keep up with discoveries is essential.
For example, image classification has seen in recent years transitions from plain convolutional networks, to the introduction of batch normalization~\cite{ioffe2015batch}, residuals~\cite{he2016deep}, inverted bottlenecks~\cite{sandler2018mobilenetv2}, and a transition to transformers~\cite{vaswani2017attention}.
A team working on image classification that wants to keep their models up to date would have had to incorporate these changes either by adapting the external code through interfaces or simply rewriting it -- both time-consuming processes.
This is challenging because different teams develop their own conventions without any unifying standards. Our paper addresses this problem by extending {\NAME}~\cite{peng2020pyglove} to a language that allows defining flexible standards and writing rules for how to use the standards to exchange code easily.

Flexibility is key, as enforcing strict standards may limit long-term progress. This is because it can be difficult to avoid over-emphasizing our current ideas when defining conventions. For example, in 2015, we may have adopted an interface in which every layer receives only the activations of the previous layer, so in 2016 we would have had to rewrite our interface to include the skip-connections of a ResNet. Another example would have been to assume independence across examples at training time, which would need to be broken to apply batch-normalization. In each case, we made an assumption that was later broken by new discoveries. One possible solution is to simply accept that standards must evolve \cite{sussman2007building}. Thus, our approach allows defining editable standards.

To achieve these goals, {\NAME} takes a rule-based approach: standards are first defined by light-weight annotations of ML code and then rules indicate how the code should be shared. For example, consider a situation in which ``team A'' maintains an image classifier and ``team B'' independently comes up with a new convolutional layer that should improve most image classifiers. In the {\NAME} approach, team A can annotate their (pre-existing) code with statements akin to ``this is a convolution'', ``this is a nonlinearity'', and so on, and team B would annotate their new layer with statements akin to ``these are hyperparameters'' (see \Secref{sec:symbolic-patching}).
Up to this point in our example, the two teams need not have interacted at all. Upon team A learning about the new layer, A can write a one-line rule equivalent to ``replace all my convolutions with team B's layer'' (technically accurate examples in \Secref{sec:symbolic-patching}).
Additionally, {\NAME} also allows a novel twist: team B can write the replacement rule themselves -- such a rule would be analogous to ``in any image classifier, replace all convolutions with our layer''. Then any team with a {\NAME}-annotated image classifier can apply the rule produced by team B. This twist opens up future collaboration options through repositories of ML inventions, which we discuss in \Secref{subsec:patch-power}.

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-5mm}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{src/figures/network_effects_v3.pdf}
  \end{center}
  \label{fig:network-effects}
\vspace{-4mm}
\caption{
Applying $m$ new ML innovations to $n$ teams leads to $n{\times}m$ new applications.
{\NAME} expresses an ML innovation as a rule and can efficiently exchange ML ideas via sharing rules.
% Network effect among ML ideas: with existing ideas (expressed by rule -- a block), introducing a new idea can lead to an exponential growth of the applications of these ideas.
%
% A single additional patching rule (\#N+1) leads to 
%
%more than O(N) different kinds of experiments.
% 6 patching rules leads to 9 unique valid object detection experiments. Adding an experiment will double the number, creating a network effect.
}
\end{wrapfigure}
PyGlove's rule-based approach is not constrained to the sharing of architectural changes but applies to all aspects of the ML pipeline, such as data augmentation, training algorithm, or meta-learning. In particular, as ML hardware improves, there is a recurring need to scale up model capacity. Empirical and theoretical rules have been invented to address this problem~\cite{sussman2007building,tan2019efficientnet,yang2021tuning}. Such rules could be broadcasted throughout an organization or the community, saving valuable engineer time.
% Moreover, network effects are possible by combining these rules.
This is true even across codebases, provided the guidelines in \Secref{subsec:scale-ml-network-effect} are followed, as shown in \Figref{fig:network-effects}.
In addition to the sharing of code, {\NAME}'s rules can also allow an individual to manipulate their ML system. In all these cases, our rule-based approach stands in contrast to current methods, which typically require multiple in-place edits that do not scale well with the size of the model or with the number of practitioners in the community.
These comparisons are detailed in \Secref{sec:pyglove-analysis}.\looseness=-1



The reason why {\NAME} can be applied broadly to all aspects of ML code -- and indeed beyond ML -- is its principled symbolic programming design~\cite{mccarthy1960recursive}.
Under this paradigm, {\NAME}-annotated Python objects become editable symbols, and {\NAME} rules are meta-programs that act on these symbols.
The rules are also symbols themselves, allowing compositionality similar to that of a LISP program's ability to self-edit~\cite{steele1990common}.
In \Secref{sec:symbolic-program-ml}, we describe symbolic programming and explain the {\NAME} design.\looseness=-1

To summarize, our contributions are:
\begin{itemize}
    \item a novel annotation-based language to express flexible standards that can evolve over time;
    \item a principled, rule-based method for easily exchanging complex ML ideas as code;
    % \item a guideline for maximizing the network effects through combining the exchanged ideas.
    \item guidelines to use {\NAME} to enable collaboration among large numbers of engineers and researchers;
    % \item a formalization of allowing programs to modify programs at runtime for ML.
    % \item a formalization of {\NAME}'s programming paradigm for ML
    \item A formulation of ML's life-cycle through a symbolic programming paradigm.
    % for machine learning.
    % \item a formalization of our method as symbolic programming for machine learning.
\end{itemize}

The final product, {\NAME}, is open-sourced with this paper.
%at GitHub \url{https://github.com/google/pyglove}.


==> src/submission/backup/submission/2_method.tex <==
\section{Expressing ML Ideas Through Patching }\label{sec:symbolic-patching}

The engineering process of ML is to journey from experiment A to experiment B, in which an iteration is made by manually applying the conceptual rules that formulate an idea to an ML program---a process of source code manipulation.
For example, supposing an ML practitioner wants to swap all the convolution layers with separable convolution layers in a neural network, the practitioner must locate the appearances of all convolution units in the model source code and replace each of them with the intended separable convolution.
To automate this process, we need the ML program to be manipulated programmatically. 
Such program modification is not only necessary to implement an idea but required to apply the same idea to other ML programs without complicating their codebases.
% A natural intuition is to allow an ML program to be dynamically modifiable at run time, which has been long offered by a symbolic programming paradigm originated from LISP~\cite{steele1990common}, later introduced to AutoML by {\NAME}\cite{peng2020pyglove}. Here we extend {\NAME}'s symbolic capacity from AutoML~\cite{peng2020pyglove} to ML, to express the rules embodied in the previous manual process and encapsulate them into reusable program units across different ML programs.
A natural intuition is to allow an ML program to be dynamically modifiable at run time. Motivated by this, we develop {\NAME} to express the rules embodied in the previous manual process and encapsulate them into reusable program units across different ML programs.
% ~\cite{hutchins1985direct}
As a result, not only a complex idea can be implemented by directly manipulating the ML programs, but also the laborious repetition of daily ML practices can be captured by such program expression of rules -- \emph{patches}.
The use case mentioned above in which team A applies team B's latest convolution invention without laborious manual coding is illustrated in \Figref{fig:symbolic_exp_sim_v1}.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\textwidth]{src/figures/patch_overview_v2.pdf}
    \includegraphics[width=0.9\textwidth]{src/figures/first_patch_simple_example_v4.pdf}
    \caption{
Team B's new invention \TT{SepConv} is developed agnostic to Team A's experiment, but its rule \TT{apply\_sepconv} can be patched to upgrade Team A's experiment into \TT{new\_resnet}.
In this code, \TT{pg.symbolize} is the annotation that adds the editable trait to regular Python classes, and \TT{pg.patch} is the operation that applies a rule to an object of an annotated class.
}
    \label{fig:symbolic_exp_sim_v1}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth]{src/figures/symbolic_exp_complex_v2.pdf}
    \caption{
Three more complex ideas are expressed via {\NAME} patching rules.
(Left) To change the dataset for a classification task, we need to change both the dataset and the model header's width to align with the number of classes.
This is done by querying the location of the last Dense layer, and returning the new value for both the dataset and the dense units associated with their locations as an update to the experiment.
(Middle) To multiply a scaling factor on the channels of the Conv and FC layer, the patching rule is defined by a function for transforming each node in the object tree, which takes the location, value and parent of current node as input, and modifies the `channels' member of Conv and FC classes. (Right) A upgraded version of previous example, which uses AutoML for scaling the model with a target FLOPs. To do so, it generates a search space of scale factors, and connects the search space to an AutoML trainer, which automatically figure out the best choices.
% based on the target flops.
}
    \label{fig:symbolic_exp_complex_v1}
\end{figure}






\subsection{The Power and Compositionality of Patching}   \label{subsec:patch-power}



\begin{wrapfigure}{r}{0.32\textwidth}
  \vspace{-6mm}
  \begin{center}
    \includegraphics[width=0.32\textwidth]{src/figures/patch_composition_v3.pdf}
  \end{center}
\vspace{-4mm}
\caption{
The LaMDA paper~\cite{thoppilan2022lamda} can be obtained by applying a composition of patches on the Transformer paper~\cite{wolf2020transformers}.
}
\vspace{-5mm}
\label{fig:patch_composition}
\end{wrapfigure}
The simplicity of {\NAME} to express rules is also applicable to more complex ideas.
With a capacity of direction manipulation~\cite{hutchins1985direct}, the user can modify program parts in an ML experiment by locations or by rules.
For example, \Figref{fig:symbolic_exp_complex_v1} illustrates how to change dataset, scale the width of neural models, and automatically scale the model by AutoML through {\NAME}.


% Patches themselves are symbolic objects \daiyip{Can we use it and refer to later section without definition?}(See \Secref{}), which can be serialized and moved across codebases and processes.

Simple patches can be combined together to express complex ideas.
For example, the recent large-scale NLP algorithm, LaMDA~\cite{thoppilan2022lamda}, can be obtained by applying common patches to the Transformer paper~\cite{wolf2020transformers}.
We briefly introduced how this can be implemented with {\NAME} in \Figref{fig:patch_composition}. 


Patches, i.e., program expression of rules, are useful not only because they make the expression of ideas straightforward but also because they can be shared freely and applied to different ML experiments.
{\NAME} allows patches themselves to be easily shared across codebases.
It allows users to create a patch from a URI-like string, which is human readable and can be easily referred to with a global unique name. For example, a patch for changing dataset to ImageNet~\cite{deng2009imagenet} can be described as \TT{``change\_dataset?name=imagenet''}.



% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-10mm}
%   \begin{center}
%     \includegraphics[width=0.45\textwidth]{xfigures/patch_network_effect_v1.pdf}
%   \end{center}
% \vspace{-4mm}
% \caption{
% 6 patching rules leads to 9 unique valid object detection experiments. Adding an experiment will double the number, creating a network effect.
% }
% \vspace{-1mm}
% \label{fig:patch_network_effect}
% \end{wrapfigure}


\begin{wrapfigure}{r}{0.58\textwidth}
  \vspace{-6mm}
  \begin{center}
    \includegraphics[width=0.58\textwidth]{src/figures/deep_network_effect_v4.pdf}
  \end{center}
\vspace{-4mm}
\caption{
Without {\NAME}, patching $m$ changes into $n$ teams requires $n\times{m}$ modifications to the code.
With {\NAME}, each $A_{i}$ team annotates their own code and each $B_{j}$ team writes their own rules.
As a result, patching all changes takes $n+m$ changes only.
}
\vspace{-8mm}
\label{fig:deep_network_effect}
\end{wrapfigure}
The compositionality of patches leads to a network effect among the ML ideas. We illustrate a common scenario in \Figref{fig:deep_network_effect}, that how research teams (Teams $B_{i}$) share their latest discoveries with product teams (Teams $A_{i}$). Based on {\NAME}, a research discovery can be encapsulated by a patching rule. Once the rule is created, any product team whose codebases are annotated by {\NAME} in a compatible way can apply it. This means that a research team's idea can be adopted by many product teams without manually integrating it each time. Similarly, a product team can try many research ideas quickly. This has not yet count the combination of patches, which can grow the degree of network effect exponentially. 


%\tododp{Revise the words to align with the new figures.}
% As illustrated in \Figref{fig:network-effects}, we have $3$ patching rules for data augmentation policies and $3$ patching rules for learning schedules.
% Then, we can get $3*3=9$ different experiments through combination, even if the learning schedules are mutually-exclusive and augmentation policies are also exclusive.
% Furthermore, when we add an experiment, for example, an image classification task, it will double the number of valid combinations. Therefore, once we have a fair amount of patching rules and experiments, the variety of valid experiments that can be expressed can grow exponentially.

% \tododxy{can you add a diagram here to illustrate the network effect described above?} # DONE

\subsection{Scaling Up the Network Effect of ML Ideas}\label{subsec:scale-ml-network-effect}

Patches need to be written wisely. For example, consider the following potential pitfall: assuming a research team has found a brilliant way to figure out the learning rate for image classifiers, they write a rule depending on a ``\TT{learning\_rate}'' property of the task after seeing it fit for an \TT{ImageClassificationTask} class.
Later someone in this team wants to apply the rule to another image classifier - \TT{ImgClsTask}, which, instead of having \TT{``learning\_rate''}, has a \TT{``lr''} property. The rule will surely fail due to the mismatch between the expected and actual locations for the learning rate. In such case, a better rule can be written as - matching any node under the task whose key is either \TT{``learning\_rate''} or \TT{``lr''}, which not only work for the cases above, but also for cases that specifies learning rate not as an immediate property of the task, but under its sub-node such as an optimizer.
This approach, however, does not scale well since the pre-defined assumptions cannot always meet the growth of heterogeneous components. As a result, to maximize the generality of rules, we need to reduce the discrepancies among ML components by advocating reuse at both the low level (e.g., network layers) and higher levels (e.g., training loop definition).

Standardization is the process of reducing the applicability issues for patching across codebases. It sounds alarming, as usually, standardization means reducing flexibility and autonomy.
In our proposal, however, we suggest an ML component ecosystem that carefully considers the flexibility and self-govern needs, while allowing different codebases to converge in what ML components they use incrementally. Such an ML ecosystem should have the following requirements:

\textbf{(1) Concept-oriented} Components in the ML ecosystem should precisely represent the concepts in the human mind. They should be able to be put together by composition and can be manipulated easily. ML components like this should allow a natural mapping of the concepts and straightforward expressions of ideas, which makes them competitive for broad adoption.


\textbf{(2) Scalable for extension} The components should be extensible without modifying the existing source code.
In other words, a component can be extended without modifying its class definition, and an object of the component should be able to be modified without changing its source code.

\textbf{(3) Runtime independence} The user-facing interfaces should be independent of the execution environment, such as ML frameworks, hardware accelerators, etc.
If so, it will allow the identical ML experiment definition to run consistently from everywhere.

\textbf{(4) Maximizing sharing} Both ML components and their objects can be easily shared. Moreover, ML objects of common interests, such as well-known experiments, can be retrieved with a globally unique identifier (e.g., URL), which automatically imports their required components.
Therefore, ML experiments and techniques can be easily referenced by their identifiers.

\textbf{(5) Adaptive to changes} The ML ecosystem needs to adapt to the rises and falls of standard components.
This requires a scalable way of upgrading the existing experiments with new components that replaces the old components.

\textbf{(6) Supporting accessibility} The advocate for sharing does not mean that everything needs to be public. Organizations or individuals are welcome to have their own assets, no matter it is IP reasons or certain assets are too early to be shared publicly. Accessibility can be controlled at both component level and object level.

{\NAME} provides solutions to all these requirements:
\begin{itemize}
    \item A PyGlove-annotated object is a straightforward solution for developing concept-oriented components, which is compositional and mutable, addressing requirement (1).
    \item A PyGlove-annotated class can be extended by subclassing, and its object can be modified with manipulation, satisfying requirement (2).
    \item Patches can be easily developed to map common PyGlove-annotated classes to their runtime-specifc versions. Therefore, the user-facing components are decoupled completely from the components for implementation, meeting requirement (3).
    \item PyGlove-annotated objects are serializable, which can be stored in a file or database. Moreover, the serialized information contains the information for importing their components, so users can load the object through a single URL, addressing requirement (4).
    \item Upgrading an old component in existing experiments can be described as a patch, which can be triggered periodically on existing experiments, meeting requirement (5).
    \item Requirement (6) can be achieved easily with existing source control solutions.
\end{itemize}

%
% \tododxy{can you please insert a figure for supporting runtime independence?}
%\subsection{An Ultimate Goal}


% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-7mm}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{xfigures/final_picture_v1.pdf}
%   \end{center}
% \vspace{-3mm}
% \caption{
% The experiment of the LaMDA\cite{} paper can be be described as a previous experiment combined with existing or new techniques.
% }
% \vspace{-6mm}
% \label{fig:final_picture}
% \end{wrapfigure}



==> src/submission/backup/submission/3_symbolic_ml.tex <==


\section{Symbolic Programming for Machine Learning}\label{sec:symbolic-program-ml}


Patching demonstrates a unique angle to view machine learning programs through a lens of symbols, which directly maps the concepts from the human mind to computer program expressions~\cite{sussman2007building}. Symbolic programming, however, has a much broader usage in the entire life-cycle of ML than just patching. Before we get to that point, let's take a brief look at what symbolic programming is, why we need it in ML, and what's PyGlove's offering about it.

Symbolic programming, which originated from \cite{steele1990common}, is a programming paradigm to manipulate its own components as if they were plain data~\cite{mccarthy1960recursive}.
Symbolic programming is interesting to ML since ML is overloaded with a constant need for modifying the source code of  ML programs.
It accommodates the ideas that can not be done with predefined interfaces and frequently changed hyperparameters. When rules are introduced to change the behavior of programs, they either need to change the source code or manipulate them at run time. The former is not viable for ML, since ML requires different experiments to be obtained from the same source code. The other option seems to be a more flexible solution to try. Have we considered code generation?
Of course, manipulation has to be done with code generation at run time. But what about generating source code?
Our answer is no.
It is neither easy nor flexible, because (1) it requires templates for the source code, which are not generally applicable to all existing code, and (2) it is difficult to accommodate complex manipulation patterns, such as mutate-run-mutate, which is commonly needed in ML. For example, in \Figref{fig:symbolic_exp_complex_v1}-1, to change the dataset for an ML classifier, we need to generate code for loading that dataset by a name, evaluate it to get the number of classes for the task, and then apply the number to generate the code of the model head width.


\subsection{PyGlove's Symbolic Programming Solution}


PyGlove formulates its symbolic programming solution through the concept of symbolic object.
A symbolic object is a unity of symbol and object, with the two aspects synchronized, meaning that \textit{a symbolic object can be manipulated as a symbol, while it can be evaluated as a regular object}.
A symbolic object is an instance of a symbolic class, which can be created by annotation \TT{pg.symbolize}, illustrated in \Figref{fig:symbolic_ops}(1). While the class can be used as a regular class, this tiny decorator makes the operations illustrated in \Figref{fig:symbolic_ops}(2-8) applicable to its objects. Symbolic object has many characteristics: first of all, the construction information (type, constructor arguments) is preserved, which defines its \emph{symbolic representation}. Such representation is identical between its source form and run-time form, thus carries necessary information to fully embody the concept that the object represents. As a result, such representation is a proxy to the concept for manipulations - ideas can be expressed as direct manipulation~\cite{hutchins1985direct} of concepts through their symbolic representations. On the other hand, a symbolic object is also a program entity that exists at run time, which carries data members and methods, behaving like a regular object. The unity of being symbolic and being an object allows a symbolic object to take advantage of the capabilities from both object-oriented programming and symbolic programming, while the former allows a modular and extensible software design, the latter brings the power of meta-programming through manipulations.


\begin{figure}[h!]
    %\vspace{-5mm}
    \centering
    \includegraphics[width=0.90\textwidth]{src/figures/ml_symboy_ops_v1.pdf}
    \caption{The definition of a symbolic class, its instance (an symbolic object), and common symbolic operations that can be applied on it. A symbolic object can be developed, validated, inspected, compared, cloned, serialized, mutated, place-held and generated with ease.}
    \label{fig:symbolic_ops}
    \vspace{-1mm}
\end{figure}



\subsection{How Symbolic Object Serves Machine Learning End-to-End}


%Now we take a breadth-first view at how PyGlove serves the life-cycle of ML. \Figref{fig:symbolic_ops} shows the symbolic operations that are used during daily ML workflows. Through \Figref{fig:ml_cycle}, we demonstrate the combination of such operations can effectively address the requirements from different phases of the ML life-cycle, from reproduction to release.

Let us take a closer look at how symbolic object serves ML.
First, the mutability of symbolic object removes the need for hyperparameter containers, which makes the development and use of ML components much simpler and more consistent. Second, the combination of symbolic operations can effectively address the need of ML experimentation with a few lines of code. \Figref{fig:ml_cycle} illustrates the symbolic operations involved in the ML life-cycle based on the \TT{MLExperiment} class defined in \Figref{fig:symbolic_ops}.\looseness=-1




\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{src/figures/ml_experiment_cycle_v4.pdf}
    \caption{
    {\NAME} serves the ML life-cycle.
    {\NAME} simplifies the engineering efforts involved from the birth of a research idea to its graduation while making the whole or parts of an experiment reusable.\looseness=-1
    }
    \label{fig:ml_cycle}
    \vspace{-5mm}
\end{figure}



Reproducing an experiment (\Figref{fig:ml_cycle}(1)) can be done by obtaining the experiment object and evaluating it (e.g. calling its \TT{train} method). Since symbolic objects are serializable, users can obtain the experiment by loading it from a file or an experiment repository.
As we have discussed in \Secref{sec:symbolic-patching} extensively, iterating an experiment (\Figref{fig:ml_cycle}(3)) involves patching the experiment with pre-existing or new components. When new components are required, symbolic components can be created similarly as regular components plus applying a \TT{pg.symbolize} decorator (\Figref{fig:ml_cycle}(2)). Although an experiment can be manually iterated by hand, it is cumbersome to run all the experiments manually, especially when the combination of modifications results in a large space of experiments to explore. Symbolic placeholding makes automatic tuning (\Figref{fig:ml_cycle}(4)) easy - by replacing the values to tune with search space specifications, concrete experiments can be generated from the space under the control of tuning algorithms. Such tuning works for both hyperparameters and neural architectures, as well as other experiment parts such as losses, optimizers, data augmentation policies, and etc. Finally, when an experiment is ready for graduation (\Figref{fig:ml_cycle}(5)), it can be serialized into a file or saved in an experiment repository. Not only the experiment as a whole, but also its parts. New components and patching rules shall also be checked in as standard ML modules.

% If a new ML component is introduced, the component needs to be made available to the consumers of the experiment. This can be done by merging back the code to the right codebase based on the access level of the experiment.


% When the user start to evolve the experiment into new ones, developing new components are usually required. With {\NAME}, new ML components can be developed as a regular class with applying a . 


% n existing experiment, changing the combination or values of existing parts, or both.
% The mutability of symbolic object makes iterations straightforward: the user can (1) cherry-pick the experiment parts and change them, for example, applying the newly introduced \TT{MaskRCNN} model to a new dataset and modifying the learning rate; (2) apply rules to modify the experiment, for example, replacing all the \TT{ReLU} layers with the \TT{SquareReLU} layers; and (3) apply encapsulated techniques without knowing the implementation details, for example, the experiment can be patched with applying three techniques illustrated in \Figref{fig:ml_cycle}: scales up the batch size and learning rate simultaneously, applies the RMSProp optimizer and turns on AutoAugment~\cite{cubuk2019autoaugment}.

%\textbf{Automatic Tuning}
% Although an experiment can be manually iterated by hand, it is cumbersome to run all the experiments manually, especially when the combination of modifications results in a large space of experiments to explore.
% Symbolic placeholding makes automatic tuning easy - by replacing the nodes to tune with search space specifications, concrete experiments can be generated from the space by tuning algorithms. Such tuning works for both hyperparameters and neural architectures, as well as other experiment parts such as losses, optimizers, data augmentation policies, and etc.

%\textbf{Release}
% Finally, when an experiment is ready for graduation, it can be serialized into a file or saved in an experiment repository. If a new ML component is introduced, the component needs to be made available to the consumers of the experiment. This can be done by merging back the code to the right codebase based on the access level of the experiment.


%Experiment parts can be created as the objects of such symbolic classes, which are also serializable thus can be shared too. Besides, symbolic comparison, diff, and visualization can improve the developer tools substantially.



==> src/submission/backup/submission/4_analysis.tex <==

\section{An Analysis of PyGlove's Approach}\label{sec:pyglove-analysis}


Behind the power of patching and the simplicity in how {\NAME} serves ML, there lies a more profound question - what is the essence of {\NAME}'s approach, and how does it compare with existing approaches in the context of ML?
We include a brief answer to this question as follows.\looseness=-1



{\NAME}'s approach to ML is focused on encapsulating the engineering efforts (e.g., modifying source code) that are involved in the journey from experiment A to experiment B. It is based on an insight that new ideas are much fewer than their applications and how they can be combined.
% Regarding developing components for new functionalities, {\NAME} does the same as the traditional approach.
PyGlove provides a unique solution for enabling flexible interfaces for ideas to be expressed, reused and shared easily.
More abstractly, {\NAME} enhances the object-oriented paradigm by adding symbolic programmability on objects, so the objects that represent ML experiments can be easily manipulated at run-time by rules, encapsulating the process of machine learning other than merely products.

\subsection{Comparison to Non-symbolic Solutions}

\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-15mm}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{src/figures/hp_container_v3.pdf}
  \end{center}
\vspace{-4mm}
\caption{
The separation of experiment representation (Left) and experiment definition (Right) in a non-symbolic ML program.
}
\vspace{-5mm}
\label{fig:hp_container}
\end{wrapfigure}
An apparent difference between {\NAME} and non-symbolic solutions lies in whether or not hyperparameter container is required to serve as a separate editable representation for a ML program, in contrast to experiment definition which are the ML components that implement the representation. In {\NAME}, an ML experiment (e.g., using Adam~\cite{kingma2015adam} to optimize a ResNet~\cite{he2016deep} model with cross-entropy loss) is represented as a symbolic object - a unity of experiment representation and definition.
While in non-symbolic solutions, since experiment definition is not directly mutable, it requires a separate editable representation as an indirection to create the experiment, illustrated in \Figref{fig:hp_container}.\looseness=-1

The separation of experiment representation and experiment definition not only causes redundancies but also introduces inconveniences due to a need for synchronization.
There are three common scenarios.
First, the developer needs to modify an component's representation when its paired definition is updated, and vice versa. Such synchronization includes but is not limited to documentation, validation rules, and logic for accommodating sub-component creations.
Second, when the user is working on an experiment representation, all automation tools that need to access its component definitions cannot simply work, such as auto-completion, code navigation, etc.
Third, when debugging a running experiment, to map the error back to the experiment representation is very difficult, especially when complex composition of the same component type is involved. For example, to identify which Conv layer has caused an input shape mismatch.

% The separation makes it difficult to encapsulate rules.
% When it comes to encapsulating rules, which is the main topic of this paper.
Encapsulating rules is difficult when the aforementioned separation exists.
This is because the separation of the two parties makes meta-programming difficult.
An example is to implement a \TT{change\_dataset} rule in \Figref{fig:symbolic_exp_complex_v1}-1.
We need to query the number of classes for that dataset, since the model head' width should be updated accordingly.
This was naturally implemented by invoking the \TT{num\_classes} property of the symbolic dataset object.
However, in a non-symbolic system, we will need to create a temporary dataset object from its representation to get the property.
% DXY: I just removed that, as I can not understand it easily.
% If this is still doable, then the following use case will be very difficult - a transformer model that requires a shared token embedder between the encoder and decoder network - this requires to break the 1:1 relationship between the definition and produced object, while through symbolic object, we can just pass the same object to two consumers.

\subsection{Caveats and Limitations}

{\NAME} employs a mutable programming paradigm, which comes with caveats and limitations.
By conventional wisdom, mutable programs are mainly criticized for three drawbacks.
(1) It is harder to program safely: since objects can change, it needs special care to ensure the program state is consistent upon mutations. (2) It is harder to reason about: downstream code may update objects created earlier; thus, it is more difficult to follow what is going on by simply looking at the code. (3) It is less performant: mutable objects need extra instructions for bookkeeping the arguments in order to handle mutation; thus, the creation of symbolic objects is slower than immutable objects. Moreover, using mutable objects for multi-threading is difficult due to the extensive locking required.
While the points are generally valid, we argue that we need to directly support it when mutability is necessary instead of being settled with a workaround.
In practice, we found that the real issues caused by mutability are rare when the program is designed properly, through extensive testing in applying {\NAME} to real-world use cases in both research and products. However, users should be informed about the run-time traits of symbolic objects.
Currently, each mutation on a tree with hundreds of sub-nodes takes only a sub-second, which might be fast enough for ML programs that train for hours or even days, but may significantly slow down programs whose evaluation takes milliseconds or less.

==> src/submission/backup/submission/5_broader_impact.tex <==

\section{Broader Impact}\label{sec:limitation}

After providing a principled solution to AutoML~\cite{peng2020pyglove}, {\NAME} takes an essential step in tackling the issues in productivity and collaborations in ML, which, in our opinion, is critical for the sustainability of ML's advancement. With providing a solution for enabling network effect among ideas in ML, together with a guideline for scaling it up to multiple codebases, {\NAME} presents an ambitious vision for enabling 10x-100x faster development of ML, by maximizing the network effects among the entire ML community - Every member in the community can easy consume and contribute to other's work, not only experiments, but also rules. With reusable rules as higher-level description of experiments, the essential contributions of research publications can be communicated precisely and effortlessly; new discoveries can generalize better through more comprehensive studies and comparisons; and the adoption can happen much faster with much less cost. On the other end, a huge efficiency boost in ML engineering would significantly reduce the engineering need for ML by eliminating redundant efforts, which may lead to a decline in the demand for ML engineers.

==> src/submission/backup/submission/6_related_work.tex <==

\section{Related Work}\label{sec:related-work}



PyGlove joins the many software libraries for ML~\cite{abadi2016tensorflow,jax2018github,paszke2019pytorch, bergstra2010theano,jia2014caffe,chen2015mxnet,wu2019detectron2, tensorflowmodelgarden2020,shen2019lingvo}, but it is the first among its kind.
Instead of adding concrete features to ML programs, it introduces a novel programming paradigm for ML by obtaining an experiment from another experiment by applying rules. As a result, not only the ideas in ML can be expressed more easily with the rules, but also can the rules be reused, shared, and combined to make a network effect among the ideas collectively.
{\NAME}'s formulation of ML engineering process is similar to the transform pipelines in compilers~\cite{bacon1994compiler, lattner2004llvm}, which take the intermediate representation (IR) of programs as input and apply transforms on top of it in chains.
The IR in {\NAME} is the symbolic representation of the object, and the transforms are the patching rules. Though similar in how they frame the problem, there are a few noticeable differences: (1) In {\NAME}, the rules are applied on the program itself, while for compilers, the transforms are applied on other programs' IR. (2) The unity of IR and execution in {\NAME} allows the modification and execution of a program to mix, which enables more dynamic run-time behaviors.\looseness=-1

{\NAME}'s solution is a type of symbolic programming~\cite{mccarthy1960recursive}. However, different from most symbolic programming solutions, such as is in LISP~\cite{steele1990common}, in which manipulations are usually done at the code definition level, {\NAME}'s solution - symbolic object - enables manipulations at the object level. As a result, it's more powerful in that it allows the same code definition to have multiple instances that can be manipulated. Also, the manipulation is safer since it operates on the binding parameters of an object, instead of the lower-level code implementations, which are usually self-sufficient. To be precise, {\NAME}'s symbolic paradigm is a mixture of symbolic programming and object-oriented programming~\cite{stefik1985object} (OOP). It allows a symbolic object to be manipulated as a symbol and evaluated as an object. Therefore, it can take advantage of the benefits of both programming paradigms - while the former allows manipulation of programs, the latter allows developing reusable components by applying the best practices of OOP through encapsulation and inheritance.\looseness=-1

Within the ML community, the most relevant work on applying symbolic programming to ML is \cite{peng2020pyglove}, which reformulates the AutoML as a process of algorithm-based symbolic manipulations. It can be viewed as a specialized application of {\NAME} in the field of ML. To extend its applicability to the broader ML, we formalize the symbolic object paradigm, emphasize the encapsulation of rules, and the network effect among them. Therefore, this paper is not a simple repetition of previous work, but an extension and generalization.\looseness=-1


% One major reason behind the rapid growth of ML in the last decade is the productivity provided by different ML libraries.
% Back to the early 2000s, researchers have to write the back-propagation for each layer in C, CUDA, or MATLAB.
% Later, Theano~\cite{bergstra2010theano}, Caffe~\cite{jia2014caffe}, MXNet~\cite{chen2015mxnet} are developed that ML practitioners can explore ideas and deploy easier.
% Following them, TensorFlow~\cite{abadi2016tensorflow}, PyTorch~\cite{paszke2019pytorch}, and JAX~\cite{jax2018github} further push the productivity for ML practitioners.
% These libraries provided basic low-level ML components, such convolution layer or optimizer.
% Upon these libraries, thousands of algorithm codebases are built to encapsulate the entire ML algorithms, such as Detectron2~\cite{wu2019detectron2} and Lingvo~\cite{shen2019lingvo}.
% Until then, exploring a new idea on an ML algorithm usually means to modify the algorithm source code.
% Such paradigm is not scalable, if you want to try it on hundreds different algorithms or ship it to tens of products.
% {\NAME} provided a principled solution to encapsulate rules (idea) and easily exchange and apply it everywhere.
% As a result, plugging {\NAME} into these the existing ML libraries/codebases can further boost the productivity to the next scale -- ultimately scaling the network effect in ML.



% The capability of {\NAME} mainly came from converting class and function into the symbolic object.
% Within the ML community, the most relevant work is \cite{peng2020pyglove}, which uses symbolic programming to program and reformulate AutoML algorithms. It can be viewed as a specialized application of {\NAME} in the field of AutoML. To extend its applicability to the broader ML, we propose to build an arbitrary ML program based on the concept of symbolic object. Therefore, this paper is not a simple repeat of previous method, but a generalization and a formalization of the symbolic paradigm.


% Symbolic object takes root in object-oriented programming and symbolic programming.
% Object-oriented programming refers to a programming paradigm based on the concept of ``objects'', which can contain data and code~\cite{stefik1985object}.
% Symbolic programming is a programming paradigm in which the program can manipulate its own formulas and program components as if they were plain data~\cite{mccarthy1960recursive}.
% The core of {\NAME} - symbolic object - benefits from both symbolic programming and object-oriented programming.
% Instead of using separate and independent entities as symbols in symbolic programming, we equip regular objects with symbolic programmability. Therefore, objects can also work as symbols, with the two aspects always synchronized during manipulations.
